Tracing and Visualizing Human-ML/AI Collaborative Processes through Artifacts of Data Work

Automated Machine Learning (AutoML) technology can lower barriers in data work yet still requires human intervention to be functional. However, the complex and collaborative process resulting from humans and machines trading off work makes it difficult to trace what was done, by whom (or what), and when. In this research, we construct a taxonomy of data work artifacts that captures AutoML and human processes. We present a rigorous methodology for its creation and discuss its transferability to the visual design process. We operationalize the taxonomy through the development of AutoMLTrace, a visual interactive sketch showing both the context and temporality of human-ML/AI collaboration in data work. Finally, we demonstrate the utility of our approach via a usage scenario with an enterprise software development team. Collectively, our research process and findings explore challenges and fruitful avenues for developing data visualization tools that interrogate the sociotechnical relationships in automated data work.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> tables/artifact_table.tex <==
\begin{table}[h!]
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
{\cellcolor[HTML]{808080}\LARGE{\textcolor{white}{\textbf{Artifact}}}} &{\cellcolor[HTML]{808080}\LARGE{\textcolor{white}{\textbf{Examples}}}} 
&{\cellcolor[HTML]{808080}\LARGE{\textcolor{white}{\textbf{Papers}}}}\\ \hline

%% Analysis Properties %%%%
\multicolumn{3}{|l|}{\cellcolor[HTML]{CCD5AE}\textbf{Analysis Properties}} \\ \hline
Analysis Type & Descriptive, Predictive,  Prescriptive & test\\ \hline
Goal & Data Problem & test\\ \hline
Source Code & Workflow, Analysis, Model Scripts & test\\ \hline

%% Data Properties %%%%
\multicolumn{3}{|l|}{\cellcolor[HTML]{CCD5AE}\textbf{Data Properties}} \\ \hline
Initial Dataset & & test \\ \hline
Wrangling recommendations & & test \\ \hline
Schema &  & test\\ \hline
EDA Insights & Lens & test \\ \hline
Descriptive Statistic & Skewness, Class Balance, Label Noise, Missingness & test\\ \hline
Contextual Augemenation & Semantic Annotations, Domain Ontologies & test\\ \hline
Benchmark Augmentation& Benchmark Datasets, Past Performance Data & test\\ \hline
Adversarial Augmentation & Noise, Ablations& test\\ \hline
Cleaning Transformations & Filtering, Grouping, Joining, Pivoting, Omitted Values& test\\ \hline
Mapping Transformation & Embedding, Encoding, Feature Maps, Basic Calculations& test\\ \hline
Splits & Train, Test, Validation, Batches& test\\ \hline

%% Model Properties %%%%
\multicolumn{3}{|l|}{\cellcolor[HTML]{CCD5AE}\textbf{Model Properties}} \\ \hline
Initial Model Specification & 
Model Choice, Initial parameter Settings, Architecture, Objective Function& test \\ \hline
Model Task  & Type, Ranking, Learned Representation& test  \\ \hline
Results  & Prediction, Classification & test\\ \hline
Feature Correlation  & Variable Correlation, Column Correlations& test \\ \hline
Feature Engineering  & Predictors, Metafeatures, Extractors, Transformations, Encodings& test \\ \hline
Important Features  & Top Predictors& test \\ \hline
Model Performance Metrics &  AUC, GINI, MCC, Cumulative Gains, Cumulative Capture, ROC Curve etc. & test\\ \hline
Model Fit Metrics  & Residuals, Calibration Methods & test\\ \hline
Model Optimization  & hyperparameters and hyperpartitions, learning rate, weight decay & test\\ \hline

%% Data Science Pipeline Properties %%%%
\multicolumn{3}{|l|}{\cellcolor[HTML]{CCD5AE}\textbf{Data Science Pipeline Properties}}\\ \hline
Pipeline Components & Analysis Stages, Model Choices, Various Modules, Topology & test\\ \hline
Pipeline  Performance Metrics & \textit{similar to model metrics} & test\\ \hline


%% Search Space Properties %%%%
\multicolumn{3}{|l|}{\cellcolor[HTML]{CCD5AE}\textbf{Search Space Properties}} \\ \hline
Search Space Algorithms& Search Space Design;  Possible Actions, various low level techniques& test\\ \hline
Search Space Summary Statistics& Search Frequencies, Trade-offs& test\\ \hline

%% Interface Components %%%%
\multicolumn{3}{|l|}{\cellcolor[HTML]{CCD5AE}\textbf{Interface Components}} \\ \hline
Pipeline Dashboards & Pipeline, Search Space& test\\ \hline
Model Dashboard& Residual Plots,Co-efficient,  ROC Curve, Assorted Visualizations,Performance Metric Table& test\\ \hline
Model Customization Interactions&Thresholds, Feature Choices, Predictor Choices, Update Initialization& test\\ \hline
Bookmarks &Shared Insights& test\\ \hline
Mark-ups &Comments, Annotations& test\\ \hline

%% User Action Properties %%%%
\multicolumn{3}{|l|}{\cellcolor[HTML]{CCD5AE}\textbf{User Action Properties}} \\ \hline
Interaction sequences & Interaction Logs, Behavioral Logs,  Interaction Rates& test\\ \hline
Behavior  Patterns & Behavior Graphs, Behavior Models& test\\ \hline

%% Automated Reporting Process %%%%
\multicolumn{3}{|l|}{\cellcolor[HTML]{CCD5AE}\textbf{Automated Reporting Processes}} \\ \hline
Automated Insight & Exploratory Data Analysis Report, Insights& test\\ \hline
Model Card & Experiment AutoDoc (From H2O.ai) & test\\ \hline
Model Report & Results Summary, Decision Recommendation& test\\ \hline

%% Analysis Properties %%%%
\multicolumn{3}{|l|}{\cellcolor[HTML]{CCD5AE}\textbf{Oversight Process}}\\ \hline
Organizational Preferences & User Preference Model, Business Values & test\\ \hline
Analysis Protocols & Model Constraints, Data Constraint & tests\\ \hline
Governance - Analyst Info & & test \\ \hline
Governance - Approver Info & & test \\ \hline
Requirements Documents & & test \\ \hline
Decision Forensics & & test \\ \hline
Key Performance Indicators &  & test\\ \hline
Analysis History & Prior Analysis, Version History& test\\ \hline

%% Computational Processes %%%%
\multicolumn{3}{|l|}{\cellcolor[HTML]{CCD5AE}\textbf{Computational Process}}\\ \hline
Environment definitions &back-end libraries; APIS, configuration files; dependency graphs& test\\ \hline
Computational Budget &Hardware Resources, Time, Min \% Completed& test\\ \hline
Computation Summary Statistics &Run-time& test\\ \hline
Semantic graph & tes& testt\\ \hline
Run-time Logs &Timestamps, Executions& test\\ \hline
Computation Plan & Model Updates, API Solvers, Queries, Proxy Tasks, Various Low-level technical details )& test\\ \hline
Benchmarks Algorithms & & test \\ \hline
Change Graph & Data, Code, Visualization& test\\ \hline

%% Computational Processes %%%%
\multicolumn{3}{|l|}{\cellcolor[HTML]{CCD5AE}\textbf{Verification Process}}\\ \hline
Drift Detection & Concept/Model/Data Drift Calculation; Drift Detection Algorithm& test\\ \hline
Drift Descriptive Statistics & Magnitude, Quantity, Type& test\\ \hline
Concept Drift Dashboard & Visualization, Characterization& test\\ \hline
Alerts & Data  Model Quality; Concept Drift& test\\ \hline
\end{tabular}%
}
\caption{Artifacts and examples elicited from AutoML toolkits, libraries, systems, and user studies. We grouped \~400 artifacts that we elicited into \artificatCat{Artifact Categories} and artifact types. Examples shown here represent individual artifacts, for brevity, not all artifacts are shown and were `rolled up' into more general descriptors, for example `Linear Regression Model' and `Random Forest' are both rolled up in `Model Choice'. Full details are available in the supplementary materials.}
\label{tab:artifacts}
\end{table}

==> tex/intro_old.tex <==
%FOCUS ON:
%This is what this technology is and what kinds of problems it solves. 
%This is how people try to understand this technology. 
%limitations of how to try to understand that tax on this technology, and then 

%frame our taxonomy relative to a higher-level example. 

\section{Introduction}

With the help of AutoML technology, data science work is increasingly more automated~\cite{Bie:AutoDS:2022}. A variety of AutoML systems, libraries, and toolkits exist \cite{Thorton:AutoWeka:2013,Olson:tpot:2016,feurer:autosklearn:2020,Zimmer:Auto-Pytorch:2021,sagemaker2020,golovin:googleVizer:2017,h202020,datarobot2020}, supporting a wide range of tasks and analytic questions. While many of these systems currently focus on the model development stage, more recent work is pushing the boundaries of AutoML to encompass a more end-to-end data science workflow~\cite{sant:automl:2021,Crisan:AutoML:2021,He:AutoML_Stota:2021,Zoller:BenchmarkAS:2021}. 


AutoML is democratizing data science work, lowering barriers to data work by reducing the necessity for deep technical knowledge of machine learning (ML) or data science (DS)~\cite{Crisan:AutoML:2021,Zequan:AlpineMeadow:2019,xanthopoulos:putting:202}. However, the automation of data science has been far from smooth. Prior research shows that, in practice, AutoML still requires considerable human labor to function~\cite{Crisan:AutoML:2021,Drozdal:trust:2020,Xin:wither_automl:2021}. Even if full automation were possible, human oversight and intervention is still desired~\cite{wang:DS_automation:2021,sant:automl:2021,Lee2019AHP,Crisan:AutoML:2021}. These studies also found that AutoML can introduce friction among an organization's teams, especially between data scientists and other team members, when it becomes difficult to audit models or analytic results. Transparent AutoML systems are essential to ease this friction. However, it is challenging to make the whole pipeline transparent to scrutiny. It is especially difficult to capture the trade-off of information between human and machine~\cite{Yang:HAI_hard:2020}.


Mechanisms exist to make AutoML systems more transparent through provenance tracking and auditing (i.e., ~\cite{Renan:ml_prov:2019,schelter:MLProv:2017,pipelineprofiler2020,wang:atmseer:2018}). These systems and others like them, have a tendency to overlook the contributions of human labor~\cite{Parasuraman2000,Horvitz:tradoff:2019,Wang:hai_collab:2019,Hong:interpret:2020,Heer:agency:2019,Crisan:AutoML:2021,Liu:Paths:2020,Xin:wither_automl:2021}. Collaboration between humans and AutoML systems, results in different degrees of automation for data science~\cite{sant:automl:2021}, which can prove difficult to follow how an analysis evolves and where potential biases, may have been introduced~\cite{Nithya:datawork:2021}. 
% Moreover, the addition of human collaboration in AutoML introduces additional complexity, forcing the systems to both \textit{evolve and adapt} in response human intervention and feedback. 
Considering this complexity, making AutoML transparent must not only account for diverse forms of collaboration across an end to end pipeline, but also the change that has occurred within the pipeline.


\textbf{To make AutoML systems more transparent and explicate the role of human labor, we propose capturing, characterizing, and tracing artifacts of data work.} In our research, artifacts represent tangible and abstract items that are generated by either humans (i.e., goals, tasks, documentation, datasets, source code, etc.) or AutoML processes (i.e, feature sets, the choice of model, automated insights, etc.). The progenitor of the artifact is a design decision of the system and the level of automation it supports. In fully automated systems, only machines generate artifacts whereas in non-automated systems only humans generate artifacts. We seek to encompass these extremes while capturing the space in between, which arises from different levels of automation~\cite{sant:automl:2021}. Research across Human Computer Interaction, Information Visualization, and the CSCW communities have attempted to capture human-machine collaboration more explicitly. This prior research proposes the design of interactive systems with varied modes of automation and information sharing~\cite{Heer:agency:2019,Hong:interpret:2020,Amershi:guidelines:2019,Yang:AutoML:2020,doshivelez:rigorous_interp:2017,zhangR:ideal_human:2021,Brent:Explain:2019,barrero:xai:2020}, including data visualization ~\cite{pipelineprofiler2020,wang:atmseer:2018,liu:mlvis_analysis:2017,zhang:ds_collab:2020} and human-in-the-loop affordances~\cite{Sperrle:EuroHILML:2020,Sperrle:HCE_STAR:2021,Endert:HIL_VisualAnalytics:2014}. However, these prior works do not suggest what pieces of the process to surface. \textbf{To address this gap, we have developed an AutoML artifact taxonomy to characterize these pieces, which we refer to as AutoML artifacts.}

Taxonomies are a widely used system of hierarchical organization that group concepts into logical associations, based on shared qualities. They provide a common language to speculate and build upon concepts. By providing a common language, taxonomies can facilitate communication within a team\cite{salmons2008expect}. Yang~\textit{et al.} note the lack of ``shared workflow, boundary objects, or a common language for scaffolding the collaboration'' make it difficult for teams with diverse skill sets to communicate and work on ML, AI, and AutoML systems together ~\cite{Yang:AutoML:2020}. Our artifact taxonomy not only characterizes these artifacts, it serves as a boundary object to provide a common language for collaboration between people with diverse and divergent skill sets.


% \revMR{
% Data science work is increasingly accomplished through the aid of automation that is made possible by AutoML technology~\cite{Bie:AutoDS:2022}. However, the automation of data science has been far from smooth. Prior research shows that, in practice, AutoML still requires considerable human labor to be functional~\cite{Crisan:AutoML:2021,Drozdal:trust:2020,Xin:wither_automl:2021}. These studies also found that AutoML can introduce friction among an organization's teams, especially between data scientists and others, when it becomes difficult to audit models or analytic results. Designing and developing AutoML systems that are transparent is essential. However, it is also challenging to capture the relevant aspects of both human and automated processes, how they interleave, and what they contribute to the final analysis~\cite{Yang:HAI_hard:2020}.
% } 

%\revMROUT{Automated machine learning (AutoML) technology lowers barriers to data work by reducing the necessity for deep technical knowledge of machine learning (ML) or data science (DS)~\cite{Crisan:AutoML:2021,Zequan:AlpineMeadow:2019,xanthopoulos:putting:202}. Beyond expanding the ecosystem of ML and DS tooling to a wider stakeholder group, AutoML is also a practical solution to the overall shortage of data scientists~\cite{sant:automl:2021}.}
% A variety of AutoML systems, libraries, and toolkits exist, including AutoWeka~\cite{Thorton:AutoWeka:2013}, TPOT~\cite{Olson:tpot:2016}, AutoSklearn~\cite{feurer:autosklearn:2020}, Auto-Pytorch~\cite{Zimmer:Auto-Pytorch:2021}, Amazon's AutoPilot~\cite{sagemaker2020}, Google Vizier~\cite{golovin:googleVizer:2017}, H20 Driverless AI~\cite{h202020}, and DataRobot~\cite{datarobot2020}. \revMR{These systems differ from prior efforts in interactive and mixed-initiative machine learning systems, which tend to be developed for a specific task. Instead, AutoML systems must support a variety of tasks and analytic questions. While many of these systems currently focus on the model development stage, more recent work is pushing the boundaries of AutoML to encompass a more end-to-end data science workflow~\cite{sant:automl:2021,Crisan:AutoML:2021,He:AutoML_Stota:2021,Zoller:BenchmarkAS:2021}. These systems can vary in complexity as they both \textit{evolve} in response to the specifics of the data and analytic tasks, as well as \textit{adapt} to human intervention~\cite{Xin:wither_automl:2021}.}

%By Yang~\textit{et al.'s} definition~\cite{Yang:HAI_hard:2020}, cutting edge and theoretical AutoML tools are \textit{evolving probablistic system}; they take on different configurations in response to new data and tasks~\cite{Yang:AutoML:2020}, but has relatively straight forward output complexity.}

%\revMROUT{These systems have different modalities for including human input and oversight. Moreover, theoretical advances in AutoML are continuously pushing the scope of these systems from their present focus on model selection and hyperparameter tuning, toward an end-to-end data science workflow encompassing preparation through to communication~\cite{sant:automl:2021,Crisan:AutoML:2021,He:AutoML_Stota:2021,Zoller:BenchmarkAS:2021}. 
%As AutoML systems continue to evolve, so to do possibilities for human input, intervention, and oversight \cite{wang:DS_automation:2021,sant:automl:2021,Lee2019AHP,Crisan:AutoML:2021}.}

% While mechanisms for provenance tracking and auditing of AutoML systems exist (i.e., ~\cite{Renan:ml_prov:2019,schelter:MLProv:2017,pipelineprofiler2020,wang:atmseer:2018}), \revMR{these systems, and others like them, have a tendency to overlook the contributions of human labor~\cite{Parasuraman2000,Horvitz:tradoff:2019,Wang:hai_collab:2019,Hong:interpret:2020,Heer:agency:2019,Crisan:AutoML:2021,Liu:Paths:2020,Xin:wither_automl:2021}. Even if full automation were possible, human oversight and intervention is still desired~\cite{wang:DS_automation:2021,sant:automl:2021,Lee2019AHP,Crisan:AutoML:2021}. This more collaborative relationship between humans and AutoML systems} results in different degrees automation for data science~\cite{sant:automl:2021}, which can make it difficult to follow how an analysis, or the creation of data product, evolves and where potential biases, or similar issues, may have been introduced~\cite{Nithya:datawork:2021}. \revMR{Moreover, the addition of human collaboration in AutoML introduces additional complexity, forcing the systems to in fact be both \textit{evolving and adapting} along with human intervention and feedback.}


%, \revMR{these focus almost exclusively on capturing the evolution of technical artifacts (i.e., paramters, model choices) and ignore. 

% Research from across Human Computer Interaction, Information Visualization, and the CSCW communities have attempted to capture human-machine collaboration more explicitly. This prior research proposes the design of interactive systems with varied modes of automation and information sharing~\cite{Heer:agency:2019,Hong:interpret:2020,Amershi:guidelines:2019,Yang:AutoML:2020,doshivelez:rigorous_interp:2017,zhangR:ideal_human:2021,Brent:Explain:2019,barrero:xai:2020}, including data visualization ~\cite{pipelineprofiler2020,wang:atmseer:2018,liu:mlvis_analysis:2017,zhang:ds_collab:2020} and human-in-the-loop affordances~\cite{Sperrle:EuroHILML:2020,Sperrle:HCE_STAR:2021,Endert:HIL_VisualAnalytics:2014}. However, these prior works do not suggest a tangible item that should be capture, traced, or visualized. \revMR{ Yang~\textit{et al.}~\cite{Yang:AutoML:2020} has also noted how prior work falls short of producing useful  boundary objects that help designers co-created effect human-ML/AI interactions alongside ML developers - whose participation is essential.}


% The  result is that systems prioritize different aspects for data work, from some focusing on specific sets of parameters (i.e., ~\cite{pipelineprofiler2020}) while others visualize a sequence of analysis steps~\cite{Liu:boba:2021}. Absent is a mechanism that can bridge across these different works to capture the broader scope of hybrid automation in data work.%
%Research in human-human collaboration and knowledge sharing has highlighted the importance of artifacts for capturing~\cite{Kreiner:tacit_artifact:2002,Lee:BO:artifacts:2007} and tracing~\cite{Tiwana:kx_system:2001,Fischer:kx_mgmt_og:2001,Mariano:kwx_mgmt_survey:2016} complex collaborative processes.

%%We take inspiration from this research to examine artifacts from the perspective of human-machine collaboration and across the continuum of automation in data work. The precise meaning of an artifact is dependent on its context. In our research, artifacts represent tangible and abstract items that are generated by either humans (i.e., goals, tasks, documentation, datasets, source code, etc.) or AutoML processes (i.e, feature sets, the choice of model, automated insights etc.) within data work. The progenitor of the artifact is a design decision of the system and level of automation it supports. In fully automated systems, only machines generate artifacts whereas in non-automated systems only humans generate artifacts. We seek to encompass these extremes, while capturing the space in between, which arises from different levels of automation~\cite{sant:automl:2021}.

%Our work focuses on captured aspects of a given process, referred to as artifacts, for knowledge transfer in human-machine collaborations. Taking inspiration from human-human collaboration, we explore the potential of artifacts as a `unit' for communicating knowledge between humans and AutoML systems. In the knowledge management and CSCW literature, artifacts are important for capturing ~\cite{Kreiner:tacit_artifact:2002,Lee:BO:artifacts:2007} and externalizing~\cite{Tiwana:kx_system:2001,Fischer:kx_mgmt_og:2001,Mariano:kwx_mgmt_survey:2016} tacit knowledge between humans. Artifacts also function as boundary objects~\cite{Star:OB_OG:1999} across domains in technical work~\cite{Lee:BO:artifacts:2007}. 

%While there do exist prior attempts to formalize and capture what could be described as AutoML artifacts from machine learning ~\cite{tateman:repo_taxonomy:2018,von_Rueden:informedml:2021,Cambronero:Software_AutoML:2021} and hybrid systems ~\cite{dellermann:future_collab:2021}. Other literature sources that do not concern AutoML directly, but do concern human-ML/AI collaboration include data science steps or primitives~\cite{Crisan:Batton:202,Heffetz:deepline:2020,pipelineprofiler2020} along with tasks\cite{dellermann:future_collab:2021,tateman:repo_taxonomy:2018,von_Rueden:informedml:2021,Sacha:Vis2ML_ontology:2019,sant:automl:2021,Renan:ml_prov:2019,Sperrle:HCE_STAR:2021,Brehmer:Typology:2013,Lam:GoalstoTasks:2018} to support artifact contextualization. The prior research landscape is rich, but it is not well integrated. In our work, we seek to build a common language across this literature, with varied degrees of automation~\cite{sant:automl:2021} at the center of this investigation. 

% \revMR{\textbf{To make AutoML systems more transparent and explicate the role of human labor, we propose identifying and capturing artifacts of data work.}} In our research, artifacts represent tangible and abstract items that are generated by either humans (i.e., goals, tasks, documentation, datasets, source code, etc.) or AutoML processes (i.e, feature sets, the choice of model, automated insights, etc.). The progenitor of the artifact is a design decision of the system and the level of automation it supports. In fully automated systems, only machines generate artifacts whereas in non-automated systems only humans generate artifacts. We seek to encompass these extremes while capturing the space in between, which arises from different levels of automation~\cite{sant:automl:2021}.

\textbf{Our research adopts a multiphased mixed methods design to first propose a taxonomy for AutoML artifacts and then investigate its utility for tracing and visualizing artifacts through a case study.} \autoref{fig:artifacts} summarizes our approach. 
\revMR{The purpose of our taxonomy is multifold. \textit{It provides a broad census of artifacts}, drawn from the literature, to provide a sense of the capabilities of AutoML systems, both existing and theoretical, and human intervention.  In creating our taxonomy, \textit{we also integrate and reconcile existing taxonomies, frameworks, and ontologies} and capture both socio- and technical artifacts.}
To develop our taxonomy, we have adopted a robust methodology that evaluates its conciseness, robustness, comprehensiveness, extensiveness, and explainability~\cite{Nickerson:taxonomy:2012,Prat:taxonomy:2015}. \revMR{We collaborate with developers of an AutoML system to create}~\SYSTEMNAME\ , a visualization prototype that shows not only individual instances of artifacts but also their creation context, dependencies, and changes over time time. \revMR{Through this case study, we demonstrate how our taxonomy can serve as a boundary object between researchers and professional development teams by enabling us to to visualize, analyze, and reflect on an existing AutoML system's design choices~\cite{Yang:HAI_hard:2020}.} Collectively, our research presents the following three contributions:


%\revMROUT{To frame our taxonomy development, we emphasize traceability as a more comprehensive way to delineate the generation of artifacts. Moreover, we provide a definition of traceability and contrast it to provenance and transparency, two common mechanisms for auditing and understanding AutoML systems. Guided by this definition, we conducted a broad examination of the literature to define a set of artifacts that are human or machine generated within automated data work. }

%We have developed an AutoML artifact taxonomy from a broad examination of AutoML systems, theoretical or otherwise, classifying artifacts that account for the human-machine hand-off of work. Moreover, 
%We take a view across the entire pipeline of data work, from data preparation to communication. 
 %\textit{Informed by prior research, we anticipate that such artifacts can occupy a broad range, from initial input datasets to parameter settings and modifications, results of analyses, to the automatic or manual construction of dashboards for communication.}
%We further assessed the ability of the taxonomy to identify and trace artifacts through a collaboration with a project team developing an AutoML system. Using APIs developed by the software development team, we identified artifacts and classified them according to our taxonomy. We then visualized those artifacts with a~\SYSTEMNAME\ -- a tool that we developed and shared with the project team. ~\SYSTEMNAME\ shows not only individual instances of artifacts but also how they depend on each other and change over time through a combination of human or machine direction. 
\begin{itemize}
    \setlength{\itemsep}{1.5pt}
    \item \textbf{A definition of traceability}, that integrates transparency, provenance, and context.
    \item \textbf{An artifact taxonomy that captures both human and machine processes in automated in data work} and that defines a set of artifacts and their properties (Section~\ref{taxonomy}).
    \item Finally, we present \textbf{AutoML Trace}, an interactive and visual sketch~\cite{greenberg:usability_eval:2008} that reifies our taxonomy and explores its utility as a boundary object for co-creating visualization tools with professional development teams (Section~\ref{prototype}). 
\end{itemize}

Our research provides timely contributions for tracing and analyzing how human and ML/AI actors work collaboratively to make decisions with data. \revMR{While we focus our research and its contributions to the challenges of automating data science, both our taxonomy and the approach we use to create it, can be used more broadly to develop frameworks and systems for designing human-ML/AI collaboration.}


\section{Traceability for Human-Machine Collaboration}\label{trace-define}

Data science is the application of statistical and computational techniques to real-world data~\cite{Crisan:Batton:202}. It comprises multiple phases, beginning with data preparation, analysis, deployment, and communication~\cite{Crisan:Batton:202}. Work carried out within these phases is growing increasingly automated and different systems vary in the level of automation they can support~\cite{sant:automl:2021,Zoller:BenchmarkAS:2021,Xin:wither_automl:2021}. 
% For example, model selection or feature generation can be carried out alternatively by humans or automated processes; work may even be initially conducted by a machine process and corrected by a human, or even vice versa~\cite{Crisan:Batton:202,Lee2019AHP,wang:DS_automation:2021,sant:automl:2021}.
Comparing the extent of automation afforded by two different AutoML systems, or even two different analyses from the same system can become complex ~\cite{sant:automl:2021}. Tracing the collaborative relationship between humans and automated processes is essential for ensuring the \textit{entire data science process is transparent and scrutinizable, not just the end product (i.e., the model or result)}~\cite{Winfield:ethics_transparency:2018}. 
% \textbf{We propose tracing artifacts resulting from data science work, from preparation to communication, achieved through hybrid modes of automation.}}

The traceability of artifacts has been explored in software and design engineering contexts~\cite{rogers:trrrace:2021,Sundaram:traceaing:2010} for some time and has more recently been explored for machine learning~\cite{mora:trace_and_trust:2021,schelter:MLProv:2017,Cambronero:Software_AutoML:2021}.% \revMR{Research in human-human collaboration also highlights the importance of artifacts for capturing~\cite{Kreiner:tacit_artifact:2002,Lee:BO:artifacts:2007} and tracing~\cite{Tiwana:kx_system:2001,Fischer:kx_mgmt_og:2001,Mariano:kwx_mgmt_survey:2016} complex collaborative processes.} However, the definitions of traceability vary widely. 
Here,\textbf{we define traceability for ML/AI as encompassing provenance, transparency, and context}. \textbf{\textit{Provenance}} is the process of recording individual artifacts and their origins; what generated the artifact and other artifacts dependent upon it. \textbf{\textit{Transparency}} concerns the ability to understand how the model arrived at its conclusions. Finally, \textbf{\textit{context}} indicates where the artifact exists with the analysis. \revMR{Here, we propose tracing artifacts from data science work, from preparation to communication, achieved through hybrid modes of automation. } We consider an artifact to be traceable if there is a clear definition of what it is, how and when it was generated, and there exists a lineage of how, if applicable, it has changed.



%\revMR{In the context of our research, the definition of data work, or more narrowly in our case of data science work, establishes the important contextual component of our defintion. Data science has had many defintions over time, with debates to its relationship data analysis more generally. We adopt a definition recently synthesized by Crisan~\textit{et. al.} that it is a \textit{``a multidisciplinary field that aims to learn new ingishgt from real-world data through the structued application of statistical and computational techniques''} and encompassing steps from data prepartion, analysis, deployment, and communication. We  strive to define, identify, and eventually collect artifacts that are generated or modified by either by humans or automated processes working collaborative and to trace their evolution over time the steps of data science work. }

%Democratizing data science is essential for enabling a variety of stakeholders to make decisions with data, as well as a practical way to address the overall shortage of data scientists. Automated Machine Learning (AutoML) technology is an important catalyst for this democratization because it  automates aspects of data science work, which enables domain experts to carry out data science work through  minimal or even no-code solutions.

%While early implementations of AutoML technologies focused on automating model selection and hyperparameter optimization ~\cite{Thorton:AutoWeka:2013}, more recent implementations of AutoML technology have broadened their scope, enabling end-to-end automation of many data science steps from data preparation, feature selection, model optimization, and finally monitoring and refinement of deployed models~\cite{sant:automl:2021,Crisan:AutoML:2021,Zoller:BenchmarkAS:2021,He:AutoML_Stota:2021}. AutoML systems, libraries, and toolkits like 

%  Though current technology allows extensive automation, human intervention and oversight are still needed. As such, a transfer of information between AutoML systems and humans is incumbent for this technology to be of practical use. 
 
% There has been growing effort to define the varied degrees of system automation and what that means for data science work~\cite{Crisan:AutoML:2021,wang:autods:2021,Lee2019AHP, Parasuraman2000}. For example, in their paper Karmaker et al.~\cite{sant:automl:2021} propose six levels of automation, from human-driven to fully automated (AutoML).
% , based upon a set of five tasks:  cleaning and curation (CDC); fitting the ML model (FML); feature engineering (FE); alternative model exploration, testing, and validation (ATV); result summary and recommendation (RSR). Their thorough analysis shows that few, if any, existing systems and toolkits achieve automation beyond Level 4, which means that some systems are capable of automating at most FML, ATV, and FE. While these steps may be fully automated and do not require human intervention, they still require human oversight~\cite{Crisan:AutoML:2021}. Systems above level 4 should also be capable of automating CDC, RSR, and TF, steps and are theoretically possible~\cite{Zoller:BenchmarkAS:2021}, though there is not a current system that does so. At present, these tasks require considerable human intervention in end-to-end AutoML systems. 
%Consequently, AutoML systems operate more as a hybrid, collaborative technology between humans and automated processes~\cite{wang:DS_automation:2021,sant:automl:2021,Lee2019AHP,Crisan:AutoML:2021,Gehrmann:SemanticInference:2020}.
% This hybrid nature makes automated data science work complicated to audit.
%The hybrid nature of these systems make for a challenging collaboration between domain experts an AutoML systems~\cite{sant:automl:2021,Qian:2018:MTeaching}. One collaboration challenge is the hand-off of information between human and machine processes. Machine learning algorithms are black-boxes. By incorporating machines into human decision-making processes via AutoML technology, it has become incumbent on the machine to explain itself~\cite{Brent:Explain:2019} and incorporate human feedback~\cite{Heer:agency:2019}. With AutoML technology automating more data science tasks, the existing problems for FML and ATV tasks, more extensively covered by prior work, are even more compounded. This in turn has led of a number of user studies and reflections geared toward the more comprehensive design of systems that support more analytic provenance and information transfer~\cite{Heer:agency:2019,Hong:interpret:2020,Amershi:guidelines:2019,Yang:AutoML:2020,doshivelez:rigorous_interp:2017,zhangR:ideal_human:2021,Brent:Explain:2019,barrero:xai:2020}.  Visualization (vis) and human-computer interaction (HCI) researchers have also made contributions to tackle these challenges through visual analytics tools, like PipelineProfiler~\cite{pipelineprofiler2020}, ATMSeer~\cite{wang:atmseer:2018}, and others~\cite{liu:mlvis_analysis:2017}, incorporate humans-in-the-loop through visualization of AutoML processes~\cite{Sperrle:EuroHILML:2020,Sperrle:HCE_STAR:2021,Endert:HIL_VisualAnalytics:2014}. However, these systems focus on the model fitting and optimization phases of the Data Science process. We found little prior work that examined human ML/AI collaboration across entire end-to-end Data Science processes utilizing AutoML technology.

% Artifacts, or captured aspects of a given process, serve as mediators in communication for human-human collaborations around data work. Leveraging this prior work in human-to-human collaborations, we advocate for surfacing artifacts captured from this hybrid process to trace and audit automated data sciences workflows, illuminating what was done, by whom, and how it affects upstream data work.
%In the space of human-to-human collaboration, artifacts or captured aspects of a process, serve as mediators in communication and a medium for transparency and traceability of what happened, when, and why \cite{zhang:ds_collab:2020,Renan:ml_prov:2019,rogers:trrrace:2021}. Here, we explore the challenges of hybrid human and AutoML systems through the construct of traceability. Inspired by research on human-to-human collaboration and knowledge sharing, we propose that an `artifact' is the primary unit of tracing knowledge and information hand-off between humans and AutoML across an end-to-end data science workflow. Prior work in this space of AutoML has considered artifacts only tangentially and primarily as generic inputs and outputs. Rather than view artifacts as by-products of automated processes, we see them as drivers of decision-making throughout automated processes.

% In our search to inform this work, we did not find any comprehensive resource to characterize artifacts and their utility in data work. From a broad examination of AutoML systems, both realized and theoretical, we define AutoML artifacts and delineate their properties through a taxonomy to fill this gap. We demonstrate the utility of our taxonomy through a collaboration with a team developing an AutoML system. Moreover, we show that surfacing and tracing artifacts can influence the design of AutoML systems that interact with humans.
%In our review of AutoML systems and literature, we found efforts to classify aspects of human-in-the-loop~\cite{dellermann:future_collab:2021} and machine learning systems~\cite{tateman:repo_taxonomy:2018,von_Rueden:informedml:2021}, that can be utilized to improve current tools and practices. These are often presented as taxonomies, a common schema for categorization and indexing of knowledge. Though existing classifications were informative for our work, we did not find a comprehensive resource characterizing artifacts (named as such or otherwise) and their utility in data work across an end-to-end analysis pipeline. Considering this, we conducted a broad examination of AutoML systems, theoretical or otherwise, classifying artifacts within a taxonomy that accounts for the human-machine knowledge transfer across the entire pipeline. Methods we employed (Section~\ref{taxonomy-method}) focused on development of a robust taxonomy that is extendable to account for future advancement in the field. In the rest of this work, we propose that it is essential to transparency, explainability, and democratization that AutoML systems explicitly extract, classify, and surface these artifacts to data workers and other stakeholders throughout an end-to-end automated data science process. \textbf{Our research concretely delineates what these AutoML artifacts are and how they may be used to augment AutoML systems and visual analytics tools that help domain experts make sense of and derive insights from their data.}


%Hybrid data work where humans and ML/AI systems collaboratively trade of tasks has been explored in prior research\cite{Parasuraman2000,Horvitz:tradoff:2019,Wang:hai_collab:2019,Hong:interpret:2020,Heer:agency:2019,Crisan:AutoML:2021,Liu:Paths:2020,Xin:wither_automl:2021}. However, these prior studies have not honed in on a element of knowledge transfer. Here we propose artifacts as a way to capture, surface, and trace these hybrid processes.

% 
% Begin last draft below
% 
% \section{Introduction}
% % Efforts to automate machine learning pipelines, referred to as AutoML, have helped democratize machine learning and alleviate the burden of entry for domain experts without data science or machine learning backgrounds.
% Democratizing data science is essential for enabling a variety of stakeholders to make decisions with data, as well as a practical way to address the overall shortage of data scientists~\cite{sant:automl:2021}. Automated Machine Learning (AutoML) technology is an important catalyst for this democratization because it  automates aspects of data science work, which enables domain experts to carry out data science work through  minimal or even no-code solutions~\cite{Crisan:AutoML:2021,Zequan:AlpineMeadow:2019,xanthopoulos:putting:202}. While early implementations of AutoML technologies focused on automating model selection and hyperparameter optimization ~\cite{Thorton:AutoWeka:2013}, more recent implementations of AutoML technology have broadened their scope, enabling end-to-end automation of many data science steps from data preparation, feature selection, model optimization, and finally monitoring and refinement of deployed models~\cite{sant:automl:2021,Crisan:AutoML:2021,Zoller:BenchmarkAS:2021,He:AutoML_Stota:2021}. AutoML systems, libraries, and toolkits like AutoWeka~\cite{Thorton:AutoWeka:2013}, TPOT~\cite{Olson:tpot:2016}, AutoSklearn~\cite{feurer:autosklearn:2020}, Auto-Pytorch~\cite{Zimmer:Auto-Pytorch:2021}, Amazon's AutoPilot~\cite{sagemaker2020}, Google Vizier~\cite{golovin:googleVizer:2017}, H20 Driverless AI~\cite{h202020}, and DataRobot~\cite{datarobot2020}, as well as others, are now widely available for use by both data scientists and other analysts.

% %  Though current technology allows extensive automation, human intervention and oversight are still needed. As such, it is incumbent on AutoML systems and humans to share knowledge for this technology to be of practical use. This hybrid nature makes automated data science work complicated to audit.
% While there is growing potential for AutoML technology to automate data science, full automation is still not possible and existing systems require varying degrees of human input and direction to function. Consequently, AutoML systems operate more as a hybrid and collaborative technology between humans and automated processes~\cite{wang:DS_automation:2021,sant:automl:2021,Lee2019AHP,Crisan:AutoML:2021,Gehrmann:SemanticInference:2020}. For example, in their paper Karmaker et al.~\cite{sant:automl:2021} propose six levels of automation, from human-driven to fully automated (AutoML), based upon a set of five tasks:  cleaning and curation (CDC); fitting the ML model (FML); feature engineering (FE); alternative model exploration, testing, and validation (ATV); result summary and recommendation (RSR). Their thorough analysis shows that few, if any, existing systems and toolkits achieve automation beyond Level 4, which means that some systems are capable of automating at most FML, ATV, and FE. However, while these steps may be fully automated and do not require human intervention, they still require human oversight~\cite{Crisan:AutoML:2021}. Systems above level 4 should also be capable of automating CDC, RSR, and TF, steps and are theoretically possible~\cite{Zoller:BenchmarkAS:2021}, but, at present, these tasks require considerable human intervention in end-to-end AutoML systems. Others have similarly proposed varying degrees of automation in data science~\cite{Crisan:AutoML:2021,wang:autods:2021,Lee2019AHP, Parasuraman2000}. A concerning conclusion from their work and others~\cite{Qian:2018:MTeaching}, is that existing AutoML systems remain challenging for domain experts to collaborate with. 

% One collaboration challenge is the hand-off of information between human and machine processes. Machine learning algorithms are black-boxes. By incorporating machines into human decision-making processes via AutoML technology, it has become incumbent on the machine to explain itself~\cite{Brent:Explain:2019} and incorporate human feedback~\cite{Heer:agency:2019}. With AutoML technology automating more data science tasks, the existing problems for FML and ATV tasks, more extensively covered by prior work, are even more compounded. This in turn has led of a number of user studies and reflections geared toward the more comprehensive design of systems that support more analytic provenance and information transfer~\cite{Heer:agency:2019,Hong:interpret:2020,Amershi:guidelines:2019,Yang:AutoML:2020,doshivelez:rigorous_interp:2017,zhangR:ideal_human:2021,Brent:Explain:2019,barrero:xai:2020}. Visualization (vis) and human-computer interaction (HCI) researchers have also made contributions to tackle these challenges through visual analytics tools, like PipelineProfiler~\cite{pipelineprofiler2020}, ATMSeer~\cite{wang:atmseer:2018}, and others~\cite{liu:mlvis_analysis:2017}, incorporate humans-in-the-loop through visualization of AutoML processes~\cite{Sperrle:EuroHILML:2020,Sperrle:HCE_STAR:2021,Endert:HIL_VisualAnalytics:2014}. However, these systems focus on the model fitting and optimization phases of the Data Science process. We found little prior work that examined human ML/AI collaboration across entire end-to-end Data Science processes, with AutoML technology automating some or all of those processes. 

% Here, we explore the challenges of hybrid human and AutoML systems through the construct of traceability. Inspired by research on human-human collaboration and knowledge sharing, we propose that an `artifact' is the primary unit of tracing knowledge and information hand-off between humans and AutoML across an end-to-end data science workflow. Artifacts, or captured aspects of a process, have been used to facilitate human collaboration and explain what happened within a given process \cite{zhang:ds_collab:2020,Renan:ml_prov:2019}.  Prior work in this space of AutoML has considered artifacts only tangentially and primarily as generic inputs and outputs. Rather than view artifacts as by-products of automated processes, we see them as drivers of decision-making throughout automated processes.
% Moreover, we propose that it is essential to transparency, explainability, and democratization that AutoML systems explicitly extract, classify, and surface these artifacts to data workers and other stakeholders throughout an end-to-end automated data science process. \textbf{Our research concretely delineates what these AutoML artifacts are and how they may be used to augment AutoML systems and visual analytics tools that help domain experts make sense of and derive insights from their data.} In service of this goal, we present the following three contributions:

% \begin{itemize}
%     \setlength{\itemsep}{1.35pt}
%     \item \textbf{A definition of traceability}, that integrates transparency, provenance, and context to support the efforts of extracting, classifying and surfacing artifacts from end-to-end AutoML processes (Section~\ref{problem-statement}).
%     \item \textbf{An AutoML artifact taxonomy} that defines a set of artifacts and their properties (Section~\ref{taxonomy}).
%     \item Finally, we present \textbf{AutoML Trace}, prototype implementation for visualizing artifacts from an end-to-end automated data science flow that spans goal definition, data preparation, modeling, deployment, and communication. We evaluate AutoML Trace with a multidisciplinary team developing an AutoML tool for domain experts (Section~\ref{prototype}). 
% \end{itemize}

% \autoref{fig:artifacts} summarizes our approach and contributions. As automation of data science work progresses, and while machine learning and artificial intelligence come under greater scrutiny, our research provides timely and actionable contributions for understanding how human and ML/AI actors work collaboratively to make decisions with data. Our research has implications for the design and implementation of AutoML systems and those that seek to visualize automated data science work.




%Prior work has investigated human expectations toward their ML/AI partners ~\cite{Horvitz:tradoff:2019,Wang:hai_collab:2019,Hong:interpret:2020,Heer:agency:2019,Crisan:AutoML:2021,Liu:Paths:2020,Xin:wither_automl:2021} and found numerous points of friction in these collaborations.

 %Increasingly, these AutoML technologies target domain experts without formal training in data science or machine learning by enabling them to leverage automation to make data science accessible to them~\cite{Crisan:AutoML:2021,Zequan:AlpineMeadow:2019,xanthopoulos:putting:202}. Moreover, there is a growing consensus that AutoML technology can help data scientists collaborate more effectively with these efforts by triaging data work to domain experts, which can remove bottlenecks for experts while also freeing up data scientists to tackle more complex questions or provide oversight and support to more domain experts simultaneously~\cite{Crisan:AutoML:2021,xanthopoulos:putting:202,Wang:hai_collab:2019}.  

%With no current AutoML system capable of fully automating an end-to-end data science process, AutoML technology requires considerable human labour and intervention to be viable~\cite{Crisan:AutoML:2021,sant:automl:2021,Lee2019AHP,wang:DS_automation:2021}. These systems are referred to as human-in-the-loop ML/AI systems. The notion of human and machine processes iterating toward a solution together is not new~\cite{Parasuraman2000}, but AutoML technology presents a unique and distinct set of challenges. Even if full automation is technically possible, a full end-to-end AutoML pipeline will likely always contain a hybrid decision-making process that trades off data work between humans and ML/AI systems~\cite{Crisan:AutoML:2021,Wang:HAI:2019}. This trade-off requires a transfer of information between humans and machines. For example, a human can provide a dataset or specify some initialization criteria, whereas an AutoML process, regardless of the level of automation, will produce some outputs for human consumption such as the final fitted model, its results, or performance metrics.





%Others have explored the role of knowledge transfer between humans and ML/AI systems~\cite{barrero:xai:2020}. They specifically propose so-called XAI, or explainable ML/AI approaches to facilitate this knowledge transfer~\cite{Brent:Explain:2019,barrero:xai:2020}. 
%In the spirit of transparency and explainability, a number of visual analytics tools, like PipelineProfiler~\cite{pipelineprofiler2020}, ATMSeer~\cite{wang:atmseer:2018}, and others~\cite{liu:mlvis_analysis:2017}, incorporate humans-in-the-loop through visualization of AutoML processes~\cite{Sperrle:EuroHILML:2020,Sperrle:HCE_STAR:2021,Endert:HIL_VisualAnalytics:2014}. However, these systems focus on the model fitting and optimization phases of the Data Science process. We found little prior work that examined human ML/AI collaboration across entire end-to-end Data Science processes, with AutoML technology automating some or all of those processes.% Winfield~\textit{et. al.}~\cite{Winfield:ethics_transparency:2018} has framed this limitation as to the tendency to focus on the final product (the ML model). They and others~\cite{Nithya:datawork:2021}, state that the present focus on ML/AI models over end-to-end processes poses a threat to the true democratization and viability of ML/AI and by extensions, AutoML, technology in practice. 

%Artifacts, or captured aspects of a process, have been used to facilitate human collaboration and explain what happened within a given process \cite{zhang:ds_collab:2020,Renan:ml_prov:2019}. In our research, we scrutinize the role of artifacts in facilitating the transfer of knowledge between human and machine processes throughout an end-to-end AutoML workflow. Prior work in this space of AutoML has considered artifacts only tangentially largely as generic inputs and outputs. Rather than view artifacts as by-products of automated processes, we see them as drivers of decision-making throughout automated processes. Moreover, we propose that it is essential to efforts of transparency, explainability, and democratization that AutoML systems explicitly extract, classify, and surface these artifacts to data workers and other stakeholders throughout an end-to-end automated data science process.
%In service of these, our research provides three contributions:


%Democratizing data science is essential for enabling a variety of stakeholders to make decisions with data, as well as a practical way to address the overall shortage of data scientists~\cite{sant:automl:2021}. AutoML technology, which automates aspects of data science work, is emerging as a viable tool to enable minimal or even no-code solutions to lower entry barriers for conducting data science work. While early implementations of AutoML technologies began to address the challenges of Combined Algorithm Selection and Hyperparameter (CASH) optimization~\cite{Thorton:AutoWeka:2013}, more recent implementations of AutoML technology have broadened their scope, enabling end-to-end automation of many data science steps from data preparation, feature selection, model optimization, and finally monitoring and refinement of deployed models~\cite{sant:automl:2021,Crisan:AutoML:2021,Zoller:BenchmarkAS:2021,He:AutoML_Stota:2021}. AutoML systems, libraries, and toolkits like AutoWeka~\cite{Thorton:AutoWeka:2013}, TPOT~\cite{Olson:tpot:2016}, AutoSklearn~\cite{feurer:autosklearn:2020}, Auto-Pytorch~\cite{Zimmer:Auto-Pytorch:2021}, Amazon's AutoPilot~\cite{sagemaker2020}, Google Vizier~\cite{golovin:googleVizer:2017}, H20 Driverless AI~\cite{h202020}, and DataRobot~\cite{datarobot2020}, as well as others, are now widely available for use by both data scientists and other analysts. Increasingly, these AutoML technologies target domain experts without formal training in data science or machine learning by enabling them to leverage automation to make data science accessible to them~\cite{Crisan:AutoML:2021,Zequan:AlpineMeadow:2019,xanthopoulos:putting:202}. Moreover, there is a growing consensus that AutoML technology can help data scientists collaborate more effectively with these efforts by triaging data work to domain experts, which can remove bottlenecks for experts while also freeing up data scientists to tackle more complex questions or provide oversight and support to more domain experts simultaneously~\cite{Crisan:AutoML:2021,xanthopoulos:putting:202,Wang:hai_collab:2019}.  

%While promising, there remain many challenges of implementing AutoML or automated data science solutions more generally. One issue that we focus on in our work is that AutoML technology continues to require considerable human labour and intervention to be viable~\cite{Crisan:AutoML:2021,sant:automl:2021,Lee2019AHP,wang:DS_automation:2021}. In practice, this means that AutoML systems have different levels of automation, depending upon their level of sophistication~\cite{sant:automl:2021}, with no system currently capable of fully automating an end-to-end data science process. These systems have been generally referred to as human-in-the-loop ML/AI systems. However, recent work has provided deeper nuance as to how much humans are actually integrated into the ML/AI Loop~\cite{sant:automl:2021,wang:DS_automation:2021,Lee2019AHP} (or if they should be~\cite{Crisan:AutoML:2021,yao:humanout:2019}). Moreover, even when full automation could be technically possible, human intervention could still be desirable to guide and audit automated data science processes ~\cite{Crisan:AutoML:2021,Wang:HAI:2019}. The result is that a full end-to-end AutoML pipeline will likely always contain a hybrid decision-making process that trades off data work between humans and ML/AI systems. For example, a human can provide a dataset or specify some initialization criteria, whereas an AutoML process, regardless of the level of automation, will produce some outputs for human consumption such as the final fitted model, its results, or some performance metrics. 

% The notion of human and machine processes iterating toward a solution together is not new~\cite{Parasuraman2000}, but AutoML technology presents a unique and distinct set of challenges. Prior work has investigated these challenges and the human expectations toward their ML/AI partners ~\cite{Horvitz:tradoff:2019,Wang:hai_collab:2019,Hong:interpret:2020,Heer:agency:2019,Crisan:AutoML:2021,Liu:Paths:2020,Xin:wither_automl:2021} and found numerous points of friction in these collaborations. Others have explored the role of knowledge transfer or fusion between humans and ML/AI systems~\cite{barrero:xai:2020}. They specifically propose so-called XAI, or explainable ML/AI approaches to facilitate this knowledge fusion~\cite{Brent:Explain:2019,barrero:xai:2020}. To emphasize the importance of shared knowledge between humans and ML/AI, Barrero~\textit{et al.}~\cite{barrero:xai:2020}  state that \textit{``XAI might enrich knowledge fusion paradigms, bringing the possibility of discovering new knowledge extractors [...] it is of paramount importance that the knowledge extracted from a model using XAI techniques can be understood and extrapolated to the domain in which knowledge extractors operate.''} In the spirit of transparency and explainability, several visual analytics tools, like PipelineProfiler~\cite{pipelineprofiler2020}, ATMSeer~\cite{wang:atmseer:2018}, as well as others~\cite{liu:mlvis_analysis:2017}, have also emerged as ways for visualizing these processes and incorporating humans-in-the-loop~\cite{Sperrle:EuroHILML:2020,Sperrle:HCE_STAR:2021,Endert:HIL_VisualAnalytics:2014}. However, we find that prior research and systems for human-ML/AI collaboration, knowledge sharing, and visual analysis, tend to focus on the model fitting and optimization parts of a Data Science process. We found little prior work that examined human ML/AI collaboration across end-to-end Data Science processes, with AutoML technology automating some or all of those processes. Winfield~\textit{et. al.}~\cite{Winfield:ethics_transparency:2018} has framed this limitation as to the tendency to focus on the final product (the ML model). They and others~\cite{Nithya:datawork:2021}, state that the present focus on ML/AI models over end-to-end processes poses a threat to the true democratization and viability of ML/AI and by extensions, AutoML, technology in practice. 


% In our research, we scrutinize the role of artifacts in facilitating the transfer of knowledge between human and machine processes throughout an end-to-end AutoML workflow. Prior work as considered artifacts only tangentially largely as generic inputs and outputs. %While prior work has arguably acknowledged the existence of artifacts, for example, by visualizing them, few have closely scrutinized the role that artifacts play in this iterative and collaborative human ML/AI (HAI) process nor the knowledge generation that results from it.
% Rather than view artifacts as by-products of automated processes, we see them as drivers of decision-making throughout automated processes. Moreover, we propose that it is essential to efforts of transparency, explainability, and democratization that AutoML systems explicitly extract, classify, and surface these artifacts to data workers and other stakeholders throughout an end-to-end automated data science process.
% In service of these, our research provides three contributions:

% \begin{itemize}
%     \setlength{\itemsep}{1.35pt}
%     \item A definition of traceability, that integrates transparency, provenance, and context to support the efforts of extracting, classifying, and surfacing artifacts from end-to-end AutoML processes (Section~\ref{problem-statement}).
%     \item An AutoML artifact taxonomy that defines a set of artifacts and their properties (Section~\ref{taxonomy}). %We derive this taxonomy from a systematic analysis (Section~\ref{taxonomy-method}) of implemented and theoretical AutoML systems. Overall, we examined approximately 400 AutoML artifacts in developing this taxonomy. Our taxonomy delineates the properties of these artifacts according to their source, whether they cross boundaries between humans and ML/AI processes, what shape they take, and finally, what tasks they support. We demonstrate how these properties help to classify artifacts.  While no one system contains all of these artifacts, by looking across a variety of end-to-end AutoML systems we anticipate that our taxonomy can accommodate future technological developments in this space.
%     \item Finally, we present AutoML Trace, a system for visualizing artifacts from an end-to-end automated data science flow that spans goal definition, data preparation, modeling, deployment, and communication (Section~\ref{prototype}). %We implement AutoML Trace in collaboration with developers of novel AutoML systems and as an evaluation of our taxonomy (Section~\ref{prototype}). 
% \end{itemize}

% As automation of data science work progresses, and while machine learning and artificial intelligence simultaneously come under greater scrutiny, our research provides timely and actionable contributions for understanding how human and ML/AI actors work collaboratively to make decisions with data. Our research has implications for the design and implementation of AutoML systems and those that seek to visualize automated data science work.

==> tex/problem_statement.tex <==
\section{Background for Problem Space and Motivation: Artifacts, Knowledge Management, and Traceability}\label{problem-statement}
This section describes relevant prior work from across disparate disciplines that demonstrate the importance of artifacts in knowledge transfer. We take inspiration from this work, and use it to define the problem space and motivation for our work in proposing artifacts' role in automated data science and within a traceability construct. 

\subsection{Knowledge Transfer between Humans and AutoML systems}\label{limit-intersection}
%people have been working with machines for a long time.
The notion of human and machine processes iterating toward a solution together is not new~\cite{Parasuraman2000}, but AutoML technology presents a unique set of challenges. Prior work has investigated these challenges and human expectations toward their ML/AI partners ~\cite{Horvitz:tradoff:2019,Wang:hai_collab:2019,Hong:interpret:2020,Heer:agency:2019,Crisan:AutoML:2021,Liu:Paths:2020,Xin:wither_automl:2021} and found numerous points of friction in these collaborations. Knowledge transfer between humans and AutoML systems is a significant challenge. Part of this difficulty stems from the `black box' nature of algorithms, referring to the  opaque internals of these models that make them difficult to scrutinize and make decisions from. However, even so-called `white box' machine learning models, whose inner workings are more readily available to analysts, can be difficult for domain experts to work with ~\cite{ocatavio:black-v-white:2019}. 

There has been a rising interest in techniques to facilitate knowledge transfer between humans and ML/AI systems called XAI, or explainable ML/AI approaches~\cite{Brent:Explain:2019,barrero:xai:2020}that seek to establish trust and greater understanding of outputs from machine learning algorithms. 
% To emphasize the importance of shared knowledge between humans and ML/AI, Barrero~\textit{et al.}~\cite{barrero:xai:2020}  state that
% \textit{``knowledge extracted from a model using XAI techniques [should] be understood and extrapolated to the domain in which knowledge extractors operate.''} 
Complimentary to this work, the visualization research community has explored frameworks, techniques, and methods for human-in-the-loop (HITL) to transfer knowledge through data visualizations~\cite{Sperrle:EuroHILML:2020,Sperrle:HCE_STAR:2021,Endert:HIL_VisualAnalytics:2014}, and these have influenced the design of visual analytics systems.

We see the primary limitation of XAI and HITL techniques is their narrow focus on the model stage of data science work and that they do not integrate the downstream data cascades~\cite{Nithya:datawork:2021} that also have a sizable impact on the outputs of AutoML processes. We acknowledge the black-box problem, but rather than focusing on interpretability and explainability like many prior works do, we explore a traceability approach. We consider AutoML processes to possess tacit knowledge of the data. Tacit knowledge typically refers to human knowledge acquired through personal or professional experience. Its importance in driving innovation within organizations has been acknowledged and widely studied by others~\cite{Suppiah:tacit_kw:2011,Lam:tacit_org:2000}. This knowledge can be derived from human pattern recognition processes that are not explicit; we consider this analogous scenario to so-called black-box machine learning models. Just as we do not need to know the connectivity of all the neurons to share knowledge with other humans, it is similarly not necessary to understand all possible weights and parameters of AutoML processes. In addition, broadening the focus from just the model to an entire end-to-end pipeline creates a highly heterogeneous collection of information to consider. We also looked to related work from outside the sphere of ML explainability to inform methods our of knowledge transfer.  

\subsection{Artifacts and Knowledge Transfer}
We reinterpret the problem of making ML/AI models transparent as knowledge sharing between human and machine processes. Among human collaborations, artifacts, or captured aspects of a process, have been found to play a critical role in capturing this tacit knowledge~\cite{Kreiner:tacit_artifact:2002,Lee:BO:artifacts:2007}. While not described as artifacts, prior research in the HCI and CSCW communities has explored ways to capture processes from data scientists to understand how they arrived at their conclusions~\cite{Mash:DSflow:2021,zhang:ds_collab:2020,Renan:ml_prov:2019}. Knowledge Management research has also extensively explored the development of systems that use artifacts to support human collaboration via the externalization of knowledge, and we draw inspiration from their insights\cite{Tiwana:kx_system:2001,Fischer:kx_mgmt_og:2001,Mariano:kwx_mgmt_survey:2016}. Importantly, artifacts externalize knowledge between humans~\cite{Fischer:kx_mgmt_og:2001} to facilitate collaboration between humans, as such, artifacts can be viewed as so-called `boundary objects' that operate between communities of practice to share knowledge and information~\cite{Star:OB_OG:1999}. In the context of our study, these two communities of practice concern AutoML processes and domain experts. In a close examination of boundary objects in computer-supported collaborative work, Lee ~\cite{Lee:BO:artifacts:2007} highlights the specific importance of artifacts to play an active negotiation role in developing a shared knowledge between these communities. 

Taking inspiration from human-to-human collaborations and knowledge sharing, we examine what it means for human and AutoML processes to transfer knowledge between them through artifacts. We believe that our approach can support existing XAI efforts by describing an additional way that humans and machines can hand off tasks and `share' knowledge, especially when that knowledge is heterogeneous. We also seek to draw artifacts from across and end-to-end data science processes with variable degrees of automation, thus extending the ability to interrogate AutoML processes beyond the model build stage. Framing machine intelligence as possessing a kind of tacit knowledge about data is potentially controversial, but we argue that it allows us to adopt a wider lens of how human and machine collaboration might exist. To the best of our knowledge, prior work has not previously explored artifacts that facilitate knowledge transfer between humans and AutoML processes.


\subsection{Surfacing and Tracing AutoML Artifacts to Address these Challenges }\label{limit-solution}

We propose traceability as a means to collect, classify, and surface artifacts from human-machine interactions that result from different levels of automation in AutoML processes. Our definition of traceability is grounded in the ideas of the tRRRace construct~\cite{rogers:trrrace:2021}, first presented in the context of visualization design studies. This construct utilizes captured artifacts from the process to trace the research conceptually and temporally. We extend the construct here toward automation in data science.  

The term traceability is overloaded. Here,\textbf{we define traceability to encompasses provenance, transparency, and context}. Many of these terms have been used interchangeably in the prior literature. We argue they are complementary but distinct. \textbf{\textit{Provenance}} is the process of recording individual artifacts and their origins; what generated the artifact and other artifacts dependent upon it. \textbf{\textit{Transparency}} concerns the ability to understand how the model arrived at its conclusions. We go further here. Instead of focusing on techniques~\cite{Harmanpreet:XAItechniques:2020} or data visualization~\cite{Chatzimparmpas:xai_vis_sruvey:2020} methods for ML models, we focus on transparency across an end-to-end AutoML process that may have different levels of automation. We treat an ML model as one of many possible artifacts that arise throughout an AutoML process and foster transparency through delineating artifacts and their properties via our proposed taxonomy. This view expands on existing XAI research, which tends to focus on the modeling steps and less on the overall process~\cite{Nithya:datawork:2021,Winfield:ethics_transparency:2018}. Finally, \textbf{\textit{context}} indicates wherein an automated data science flow the artifact exists and what affordances it offers.  We use prior research of data science steps or primitives~\cite{Crisan:Batton:202,Heffetz:deepline:2020,pipelineprofiler2020} along with tasks\cite{dellermann:future_collab:2021,tateman:repo_taxonomy:2018,von_Rueden:informedml:2021,Sacha:Vis2ML_ontology:2019,sant:automl:2021,Renan:ml_prov:2019,Sperrle:HCE_STAR:2021,Brehmer:Typology:2013,Lam:GoalstoTasks:2018} to support artifact contextualization for traceability. 

We examine ways to surface and trace AutoML artifacts to support a medium of shared understanding between human and AutoML processes. We focus on the unit of information transmitted in the form of artifacts generated by human and machine collaborations.\textbf{ In this research, we sought to delineate \textit{what these artifacts are}, \textit{how they may be characterized}, and importantly, how they may be used to trace the evolution of insights resulting from the human-machine collaboration, with different degrees of machine automation.} These aspects are detailed within our taxonomy for AutoML artifacts, which seeks to build a common language for the varied body of artifacts emergent from different AutoML systems with various degrees of automation.


% Traceability}\label{problem-statement}
% This section describes relevant prior work from across different disciplines that demonstrate the importance of artifacts in knowledge transfer. We take inspiration from this work to propose artifacts' role in automated data science processes and within a traceability construct.
% %In this section, we describe the challenges stemming from different levels of automation in AutoML processes and their effect on how these processes are successfully embedded within human decision-making and organization practices. Inspired by prior work in human-human collaborations, we motivate the importance of artifacts for sharing knowledge across the boundary of human and automated machine processes. Finally, we present a definition for traceability that scaffolds the integration of artifacts into these human-machine collaborations in automated data science work. o

% \subsection{Knowledge Transfer between Humans and AutoML systems}\label{limit-intersection}
% The notion of human and machine processes iterating toward a solution together is not new~\cite{Parasuraman2000}, but AutoML technology presents a unique and distinct set of challenges. Prior work has investigated these challenges and human expectations toward their ML/AI partners ~\cite{Horvitz:tradoff:2019,Wang:hai_collab:2019,Hong:interpret:2020,Heer:agency:2019,Crisan:AutoML:2021,Liu:Paths:2020,Xin:wither_automl:2021} and found numerous points of friction in these collaborations. In parallel with those studies,  others have explored techniques for knowledge transfer or fusion between humans and ML/AI systems~\cite{barrero:xai:2020}. They specifically propose so-called XAI, or explainable ML/AI approaches to facilitate this knowledge fusion~\cite{Brent:Explain:2019,barrero:xai:2020}. To emphasize the importance of shared knowledge between humans and ML/AI, Barrero~\textit{et al.}~\cite{barrero:xai:2020}  state that %\textit{``XAI might enrich knowledge fusion paradigms, bringing the possibility of discovering new knowledge extractors [...] it is of paramount importance that the knowledge extracted from a model using XAI techniques can be understood and extrapolated to the domain in which knowledge extractors operate.''}. 
% \textit{``knowledge extracted from a model using XAI techniques [should] be understood and extrapolated to the domain in which knowledge extractors operate.''} The visualization research community has explored frameworks, techniques, and methods for human-in-the-loop (HITL) to transfer knowledge through data visualizations~\cite{Sperrle:EuroHILML:2020,Sperrle:HCE_STAR:2021,Endert:HIL_VisualAnalytics:2014}, and these have influenced the design of visual analytics systems.

% The difficulty of sharing knowledge between humans and AutoML systems stems from the `black box' nature of algorithms, which roughly means that it is difficult for people to scrutinize the internals of these models and make decisions. However, even so-called `white box' machine learning models, whose inner workings are more readily available to analysts, can be difficult for domain experts to work with~\cite{ocatavio:black-v-white:2019}. Moreover, we see the primary limitation of XAI and HITL techniques is that they focus more narrowly on the model stage of data science work and do not integrate the downstream data cascades~\cite{Nithya:datawork:2021} that also have a sizable impact on the outputs of AutoML processes.

% We acknowledge the black-box problem, but rather than focusing on interpretability and explainability like many prior works do, we explore a complementary traceability approach. We consider the AutoML processes to possess tacit knowledge of the data. Tacit knowledge typically refers to human knowledge acquired through personal or professional experience. Its importance in driving innovation within organizations has been acknowledged and widely studied by others~\cite{Suppiah:tacit_kw:2011,Lam:tacit_org:2000}. This knowledge can be derived from human pattern recognition processes that are not explicit; we consider this analogous scenario to so-called black-box machine learning models. Just as we do not need to know the connectivity of all the neurons to share knowledge with other humans, it is similarly not necessarily to understand all possible weights and parameters of AutoML processes.


% \subsection{Artifacts and Knowledge Transfer}
% We reinterpret the problem of making ML/AI models transparent as knowledge sharing between human and machine processes. Among human collaborations, artifacts have been found to play a critical role in capturing this tacit knowledge~\cite{Kreiner:tacit_artifact:2002,Lee:BO:artifacts:2007}. While not described as artifacts, prior research in the HCI and CSCW communities has explored ways to capture processes from data scientists to understand how they arrived at their conclusions~\cite{Mash:DSflow:2021,zhang:ds_collab:2020,Renan:ml_prov:2019}. Knowledge Management research has also extensively explored the development of systems that use artifacts to support human collaboration via the externalization of knowledge, and we draw inspiration from their insights\cite{Tiwana:kx_system:2001,Fischer:kx_mgmt_og:2001,Mariano:kwx_mgmt_survey:2016}. Importantly, artifacts externalize knowledge between humans~\cite{Fischer:kx_mgmt_og:2001} to facilitate collaboration between humans, as such artifacts can be viewed as so-called `boundary objects' that operate between communities of practice to share knowledge and information~\cite{Star:OB_OG:1999}. In the context of our study, these two communities of practice concern AutoML processes and domain experts. In a close examination of boundary objects in computer-supported collaborative work, Lee ~\cite{Lee:BO:artifacts:2007} highlights the specific importance of artifacts to play an active negotiation role in developing a shared knowledge between these communities. 

% In taking inspiration from human-to-human collaborations and knowledge sharing, we examine what it means for human and AutoML processes to transfer knowledge between them through artifacts. We believe that our approach can support existing XAI efforts by describing an additional way that humans and machines can hand off tasks and `share' knowledge. We also seek to draw artifacts from across and end-to-end data science processes with variable degrees of automation, thus extending the ability to interrogate AutoML processes beyond the model build stage. Framing machine intelligence as possessing a kind of tacit knowledge about data is potentially controversial, but we argue that it allows us to adopt a wider lens of how human and machine collaboration might exist. To the best of our knowledge, prior work has not previously explored artifacts that facilitate knowledge transfer between humans and AutoML processes.


% \subsection{Surfacing and Tracing AutoML Artifacts to Address these Challenges }\label{limit-solution}

% We propose traceability as a means to collect, classify, and surface artifacts from human-machine interactions that result from different levels of automation in AutoML processes. %There exist many notions of traceability in the research literature and beyond. 
% Our definition of traceability is grounded in the ideas of the tRRRace construct~\cite{rogers:trrrace:2021}, first presented in the context of visualization design studies, which we extend here toward automation in data science. %This construct outlines three primary research tasks for conducting and reporting on design-oriented research; recording, reflecting, and reporting.  We see parallels to the challenges of trrracing artifacts in research processes to those challenges at the intersection of Human ML/AI collaboration. Here, we generalize the tasks from the tRRRace construct to more tightly integrate with Data Science and AutoML.

% There exist different definitions and meanings for traceability. Here,\textbf{we define traceability to encompasses provenance, transparency, and context}. Many of these terms have been used interchangeably in the prior literature. We argue they are complementary but distinct. \textbf{\textit{Provenance}} is the process of recording individual artifacts and their origins; what generated the artifact and other artifacts dependent upon it. \textbf{\textit{Transparency}} concerns the ability to understand how the model arrived at its conclusions. We go further here. Instead of focusing on techniques~\cite{Harmanpreet:XAItechniques:2020} or data visualization~\cite{Chatzimparmpas:xai_vis_sruvey:2020} methods for ML models, we focus on transparency across an end-to-end AutoML process that may have different levels of automation. We treat an ML model as one of many possible artifacts that arise throughout an AutoML process and foster transparency through delineating artifacts and their properties via our proposed taxonomy. This view expands on existing XAI research, which tends to focus on the modeling steps and less on the overall process~\cite{Nithya:datawork:2021,Winfield:ethics_transparency:2018}. Finally, \textbf{\textit{context}} indicates wherein an automated data science flow the artifact exists and what affordances it offers.  We use prior research of data science steps or primitives~\cite{Crisan:Batton:202,Heffetz:deepline:2020,pipelineprofiler2020} along with tasks\cite{dellermann:future_collab:2021,tateman:repo_taxonomy:2018,von_Rueden:informedml:2021,Sacha:Vis2ML_ontology:2019,sant:automl:2021,Renan:ml_prov:2019,Sperrle:HCE_STAR:2021,Brehmer:Typology:2013,Lam:GoalstoTasks:2018} to support artifact contextualization for traceability. 

% We examine ways to surface and trace AutoML artifacts to support a medium of shared understanding between human and AutoML processes. We focus on the unit of information transmitted in the form of artifacts generated by human and machine processes.\textbf{ In this research, we sought to delineate \textit{what these artifacts are}, \textit{how they may be characterized}, and importantly, how they may be used to trace the evolution of insights resulting from the human-machine collaboration, with different degrees of machine automation.}

%AutoML pipelines can also contain different levels of automation, from fully automated, which requires minimal human input toward a hybrid collaborative mode between humans and automated processes~\cite{wang:DS_automation:2021,sant:automl:2021,Lee2019AHP,Crisan:AutoML:2021,Gehrmann:SemanticInference:2020}.  One of the challenges in the hand-off of information between human and machine processes is that machine learning algorithms are black-boxes. By incorporating machines into human decision making processes via AutoML technology, it has become incumbent on the machine to explain itself~\cite{Brent:Explain:2019} and incorporate human feedback~\cite{Heer:agency:2019}. This in turn has led of a number of challenges toward the design of systems to enable this hand-off~\cite{Heer:agency:2019,Hong:interpret:2020,Amershi:guidelines:2019,Yang:AutoML:2020,doshivelez:rigorous_interp:2017,zhangR:ideal_human:2021,Brent:Explain:2019,barrero:xai:2020}. 

%Karmaker et al.~\cite{sant:automl:2021} suggests six levels for automation that delineate steps : cleaning and curation (CDC); fitting the ML model (FML); feature engineering (FE); alternative model exploration, testing, and validation (ATV); result summary and recommendation (RSR). Their thorough analysis shows that there exist few, if any, existing systems and toolkits that achieve automation beyond Level 4, which means that some current systems are capable of automating at most FML, ATV, and FE; however, while these steps may be fully automated, they may still require human oversight~\cite{Crisan:AutoML:2021}. Systems above level 4 should also be capable of automating CDC, RSR, and TF, steps, but, at present these tasks require human intervention in end-to-end AutoML systems.  Wang et al.~\cite{wang:DS_automation:2021} suggest similar levels of automation that differentiate between human directed and system-directed automation, which they describe within a larger human-in-the-loop AutoML framework. 







==> tex/prototype.tex <==

\section{Case Study with an Enterprise Development Team}\label{prototype}
% In this section, we describe an evaluation of our AutoML artifact taxonomy. We reify our taxonomy as a prototype called~\SYSTEMNAME~. For evaluative purposes, our~\SYSTEMNAME\ is a high-fidelity interactive sketch, according to Greenberg and Buxton's definition~\cite{greenberg:usability_eval:2008} definitions, that we use to assess the robustness of our taxonomy, but also its limitations.  As with prior sections, we use the \texttt{{[SM1-\#]}} notation to link to individual items of the supplementary materials that support our evaluation.
%In this section, we describe our prototype ~\SYSTEMNAME~ as a case study in the application of our taxonomy. ~\SYSTEMNAME\ is a high-fidelity interactive sketch, according to Greenberg and Buxton's definition~\cite{greenberg:usability_eval:2008} definitions. As with prior sections, we use the \texttt{{[SM1-\#]}} notation to link to individual items of the supplementary materials that provide more detail.

We conducted a case study that identified, classified, and visualized artifacts from an AutoML system created by an enterprise team of designers, developers, and project managers. \revMR{We use our taxonomy as a boundary object~\cite{Yang:HAI_hard:2020} to negotiate between our design goals of exploring traceability with their existing system and the knowledge and technical specifications of their system. As a result of this formative assessment,} 
\revMROUT{The goal of this case study was to reify the abstractions of our taxonomy and demonstrate its descriptive and comparative capabilities in a real-world setting.}

% -- a high-fidelity interactive sketch that, in the words of Greenberg and Buxton~\cite{greenberg:usability_eval:2008}, aims to  \textit{``make vague ideas concrete, reflect on possible problems and uses, discover alternate new ideas and refine current ones.''} 

%We present high-fidelity interactive sketch~\cite{greenberg:usability_eval:2008} called~\SYSTEMNAME~that helps to reify many of the abstract ideas of our taxonomy and anticipate future paths forward, but also limitations, of our approach. We present~\SYSTEMNAME~through a collaboration with developers and designers creating an AutoML system and evaluate how the surfacing and tracing of artifacts can influence the design of such systems. 

%\subsection{Prototype Goals}
%We developed a data visualization prototype~\SYSTEMNAME~to illustrate the application of our taxonomy. 
%evaluate the utility of our AutoML taxonomy. 
%We developed this visualization prototype together with a team that was developing an end-to-end AutoML system. Ultimately, we want to provide a detailed case study to illustrate how artifacts support domain experts use AutoML systems with different degrees of automation. 
% However,  there first needs to exist an AutoML system with a suitable level of automation across end-to-end data science workflows, beginning in data preparation through to deployment and communication of data products. As Karmaker~\textit{et al.}~\cite{sant:automl:2021} summarized, there exist few systems today that add automation across the six data science tasks they identified. Systems capable of greater automation and hand-off between humans and AutoML processes do not currently exist, but are under development (Section~\ref{related_work}). 
%Our AutoML artifact taxonomy can influence the design of such systems and inform how workflows conducted with these systems can be understood, as it creates a standard vocabulary to communicate, compare, and speculate.

% Our assessed if it was feasible for others to use our taxonomy to inform the development of an AutoML system. 
%Our goals with~\SYSTEMNAME\ are formative and aim to elicit how designers and developers of AutoML systems can operationalize our taxonomy. For the purposes of brevity, we refer to designers and developers of an AutoML systems as \textit{end-users} of~\SYSTEMNAME. 
%Our~\SYSTEMNAME~visualization prototype intends to surface artifacts to developers and designers to help them reflect on their system. 
%Importantly, we wanted to prompt these individuals to see and understand their AutoML system in a way that was not previously possible. 
% The~\SYSTEMNAME~prototype is not analogous to ATMSeer or PipelineProfiler, but it is complementary in providing an overview of the artifacts captured or generated by those systems. 
%\textbf{Taken together, the goal of our prototype is to elicit questions more than intends to answer specific questions participants had.}

\subsection{Collaboration Context}

\vspace{-5mm}
\revMR{\subsubsection{Overview of the existing system.} Their AutoML systems could automate aspects of data work from preparation to deployment (Section~\ref{trace-define}), including surfacing automatically surfaced insights for exploring data, feature generation, and automated model selection.  A graphical user interface (GUI) guided end-users through the analysis and revisions of the results. The end-user could intervene to modify the analysis, for example, change the model type,  via input widgets and interactions through the GUI. Certain aspects of the system also required explicit human input \textit{before} initiating an automated process. For example, the systems would surface multicollinearity (in a non-technical manner) and required that the end-user confirm which features to remove from the analysis. The end-users could deploy a model to be used by others; automated processes would also monitor for concept drift and, if necessary, alert the end-user to trigger updates. }
%Our collaborators were developing an AutoML system comprising a pipeline and a graphical user interface. They had implemented an earlier version of the system and were exploring expansion of its capabilities. The AutoML system they were developing automated aspects of the process, from data cleaning and curation to automatic reporting. However, human inputs were still required to initialize or review these processes. Humans could also override decisions made by the AutoML tool. The back-end API captured many of these human and machine-made decisions and surfaced some of these details via a graphic user interface (GUI). The GUI was the primary medium for information exchange; automated processes would generate text or visual reports for the human to review. The human would provide feedback, via input widgets and interactions, through the GUI.
%Though automated, a human could always override the defaults or provide new input. 

\vspace{-5mm}
\revMR{\subsubsection{Team composition and collaboration goals.} Our collaboration had two primary goals. First, for the team to reflect on their existing system with a better understanding of what AutoML systems are capable of. Our taxonomy created an avenue for this reflection by providing a structured vocabulary to describe their system and compared it to others. The second goal was to examine what the addition traceability would add to their system.}
 %The overall goal of our collaboration was to examine to what extent and in what ways it was possible to trace analysis 
The project team constituted a mixture of software engineers, designers, users researchers, and a project manager. Except for the project manager, the other members of the team did not have formal training in machine learning or data science. The team worked together to contextualize different components of AutoML work and implement the system.

%We approached the team with a proposal to identify, classify, and visualize artifacts stemming from their AutoML processes and using our taxonomy. 
%The front-end of their system allowed an analyst to review and interact with aspects of the pipeline through a graphical user interface.
% with the AutoML artifacts. 
% For example, the analyst could review and then agree or disagree with automatically generated suggestions for data cleaning. They could also re-run a specific model or initiate a model tournament to choose a model.
%In addition, the team developed APIs that enabled access to potential artifacts from  AutoML workflow via (mostly) public endpoints.  

%We collaborated with the team for over three months to understand their system and develop~\SYSTEMNAME. The goal of collaboration was to help the team retrospectively examine the affordances of their current AutoML and the one they had planned to develop. %In turn, this retrospective examination also motivated discussion of what their AutoML system \textit{should} support. 
%Through discussion with collabortors, we 
%Questions from our collaborators emergent from the feedback sessions were ``What downstream artifacts are affected when a given artifact changes?'', ``How do we show when a user gets a recommendation and does not take it?'', ``When do artifacts change, how, and how often?''

%was to help the team review and reflect on the system that they were developing.

%We had access to their system and could run analyses with different degrees of automation. 
% In its present use~\SYSTEMNAME~is intended as a design support tool. While aspects of~\SYSTEMNAME~could also eventually be incorporated into the AutoML system and made available to analysts 

%Surfaced within our prototype, our taxonomy helped our collaborators retrospectively examine the affordances of their AutoML system as they were developing it. In turn, this retrospective examination also motivated discussion of what their AutoML system \textit{should} support. Questions from our collaborators emergent from the feedback sessions were ``What downstream artifacts are affected when a given artifact changes?'', ``How do we show when a user gets a recommendation and does not take it?'', ``When do artifacts change, how, and how often?''
%Design and development of the \SYSTEMNAME~Interface was a highly iterative process, informed by feedback from the team we collaborated with. This team consisted of UX designers and researchers, developers, and project managers who are developing a larger system for production. This project informed the workflow we used as a basis for our design. The design process began upon completing the taxonomy development, drafting the necessary tasks, and subsequent design specifications. Design ideation began as sketches and illustrator mock-ups. Regular check-ins with the team provided feedback on the designs to narrow the design scope and make the interaction with the system more intuitive. Motivation for the final interface design was not only to address our defined requirements, but also demonstrate \textit{how} we can surface these artifacts to better understand the evolution of an analysis pipeline, see the interconnected influence of the pieces of this pipeline, and support collaboration of team members working on disparate parts.

%Developing a visualization for artifacts generated by an end-to-end AutoML pipeline is challenging. Not only are existing visual tools for doing so constrained (see Section~\ref{related_work}), but, to our collaborators, the idea of AutoML artifacts was also new. As such, there was no clear set of tasks or goals that our collaborators felt the~\SYSTEMNAME~should support. Instead, our collaborators were interested in seeing what affordances surfacing and tracing AutoML artifacts could provide. A visualization tool that allowed them to make a preliminary assessment of artifacts could them help them to form crisper goals for what more fully featured system should be able to do in the future; indeed such questions did begin to arise as we neared the completion of~\SYSTEMNAME~prototype. 

%We believe this ambiguity toward the utility of artifacts provides an optimal opportunity to evaluate our taxonomy in a real world context. Namely, can we demonstrate that our taxonomy enables our collaborators to assess Automated Data Science processes in a way that was previously not available them and also is useful.

\subsection{Identifying and Classifying Artifacts}\label{prototype-annot}
%\revMR{We identify and classify artifacts produced by the existing AutoML system by examining the outputs of its APIs.}
%The project team gave us access to a test instance of their AutoML system to experiment with. Moreover, we had access to the system's artifacts, which we classified using AutoML artifact taxonomy, via the system's APIs. 

\subsubsection{Generating Artifacts}
Within the GUI environment of the AutoML system, we created an end-to-end data analysis. We began with preparation and concluded with communication. 
% We primarily used the systems defaults in the first iteration without applying any human interventions.
%For generating the artifacts used in \SYSTEMNAME we conducted an end-to-end analysis using out collaborators' AutoML system.
% We conducted an analysis using our collaborators' AutoML system.  This analysis began with goal setting and concluded with outputting automated data insights and model results into a document where others could comment on them.  
% Through this end-to-end analysis process, there were varying points where the system made a decision automatically, others where it required input from the human before proceeding, and finally, others that were human-initiated. For example, specifying a goal was entirely human-initiated, data cleaning required human approval to apply automatically-generated recommendations, and finally, feature engineering 
During this process, we returned to earlier steps and made modifications. For example, we did not initially apply automatic data cleaning recommendations but did so in a subsequent iteration. We also let the system pick features for the model in the first iteration and subsequently changed them. Carrying out this analysis had three goals. First, to produce a variety of possible artifacts, second, to document dependencies between artifacts, and finally, to observe how artifacts change in response to user interactions. The result was a set of artifacts derived from the same analysis that changed over time.

\subsubsection{Collecting Artifacts}\revMR{We used APIs developed by the team to collect a set of JSON files our analysis. We used the API outputs over other approaches (i.e., usage logs) because these outputted the entire artifact, making it easier for us to classify the artifact according to our taxonomy. We additionally stored the order in which objects were created and could establish the dependencies of artifacts (Section~\ref{chronology-dependencies}). Like many existing AutoML systems, they did not explicate any human involvement. We had to manually record when an artifact was generated or modified by human intervention needed.}

In the infrequent instances where the  did not capture all aspects of the analysis, but we deemed an artifact was important, 
%. For example, we could not extract specifications for visualizations or user interaction logs. In some instances, 
we took a screenshot for the artifact. For example, some of the automatically generated insights for data exploration had visualizations that could not be extracted from the APIs, so we took screenshots instead. 

%For example, where we could not, as was the case with interaction logs, we indicated that the artifact had no originator. Note that the structure of the APIs did not neatly conform to our definitions of data science processes. These we classifications that we imposed on the stages of analysis.


\subsubsection{Classifying Artifacts} We annotated the files from the API calls or screenshots using our artifact taxonomy. 
% \revMR{Often, a single API output would comprise multiple artifacts, for example, the model API output would also contain artifacts pertinent to feature generation.}
%The authors reviewed and annotated sections of the files that pertained to different artifacts. Sometimes, a single file corresponded to a single artifact; for example, an API call for the model coefficients returned simply that. 
However, in most instances, a single file contained multiple artifacts. For example, an API call for information on the initial dataset returned this information along with information on recommended wrangling transformations. \revMR{The authors first \textit{identified artifacts} from these APIs by manually inspecting them in a simple development environment - demarcating and marking up instances of artifacts. Next, the authors examine each of the artifacts individually and \textit{classified them according to our taxonomy}, modifying their properties as was pertinent to analysis (i.e., whether it was human or automatically generated). Finally, we examined and recorded the dependencies amongst artifacts. The authors repeated these two steps until they reached a consensus on the artifact type and its properties; we also engaged with our collaborators to verify that our artifacts were accurate.}
%We otherwise used the same approach described in Section~\ref{taxonomy-method} to identify and classify artifacts according to our taxonomy. The annotation process was iterative and involved consultations with our collaborators to clarify the interpretation of different elements of the files. 
A final list of artifacts and their taxonomic annotations is available in~\suppDesignSpec; this list served as a backbone of our~\SYSTEMNAME~implementation. 
% \revMR{Although this was largely a manual process, we believe it can be carried out automatically in future iterations.}

\subsection{Feedback and Question Elicitation}\label{prototype-feedback}
\revMR{As a final step, we presented~\SYSTEMNAME~to our collaborators via chauffeured demonstrations~\cite{lloyd:chauffered_demo:2011} conducted over video conferencing platforms.}
%Throughout the development of~\SYSTEMNAME~, we conducted chauffeured demonstrations~\cite{lloyd:chauffered_demo:2011} with our collaborators. These demonstrations took place over virtual video conferencing platforms. 
The authors demonstrated the functionality and affordances of~\SYSTEMNAME~and our collaborators were given opportunities to provide feedback. \revMR{We iterated between discussing the analysis we conducted using their existing platform and the artifacts we harvested and visualized via~\SYSTEMNAME. This was an important step in our assessment, as it reinforced to our collaborators that traceability could be added to their existing system, as all artifacts of a real analysis were captured through their APIs. The team was excited to view not only their artifacts but, their system's capabilities, in this way.}

There was no expected structure to the feedback, nor did we have \textit{a priori} prompts for feedback. We were interested in collecting the types of questions our prototype would elicit during these feedback sessions. The engagement was dynamic, with both the authors posing and responding to questions about the artifacts, their sources, dependencies, and changes over time. What our collaborators appreciated most was being able to see their system laid out according to our taxonomy. This new view of their system led them to examine aspects of their work from a perspective that they had not previously considered. We summarize our discussion into three common themes: seeing and describing dependencies; comparing sequences analyses over time; and comparing how their system differed from others.

\vspace{2mm}
\noindent\textbf{Seeing and describing dependencies.} \revMR{Visualizing the dependencies of individual artifacts and the different types of artifacts} was something they had not been previously able to do. \revMR{They were especially interested and excited to see how the human and machine-generated processes interleaved through the analysis. This combination of the origin and dependency view allows them to infer} potential causal relationships between an artifact's current state and other actions. As we have previously indicated, many AutoML systems do not explicate the role of humans, but, with~\SYSTEMNAME\ the impact and effect of the human's role are undeniable. \revMR{The team saw the benefit of visualizing the analysis in this way as a way to reflect on the system's design. They also saw the benefit of surface such relationships to support governing an analytic pipeline. For example, if authorization is required to deploy a model, they saw~\SYSTEMNAME\ as a useful way to audit the existing analysis to either recommend or decline deployment.}

%Showing artifact Sources in context allowed analysts to trace the trade-off between human and automated processes, which was something they had not been previously able to do with their system. As they dug into individual artifacts and dependencies, our collaborators wanted to see potential causal relationships between an artifact's current state and other actions. For example, if someone commented on a model report that influenced a data scientist to retrain the model, then our collaborators wanted to trace this relationship explicitly. Another example is if an alert is generated because the system detected conceptual drift, then our collaborators wanted to dig into the sequence of events that led to this alert. Our dependency view supports this functionality but still requires additional tailoring to address the full scope of what our collaborators wanted to see. 

\vspace{2mm}
\noindent\textbf{Comparing sequences of analyses analyses.} 
%Our collaborators could immediately see how ~\SYSTEMNAME~, structured using our taxonomy, could surface and trace artifacts. 
\revMR{Our collaborators were also interested in using~\SYSTEMNAME\ to compare analyses conducted by multiple analysts over time. They specifically wanted to have multiple analysis sequences generated by different actors and to compare them. This scenario of asynchronous human collaboration, together with individual human-machine collaboration, is a promising sign of our taxonomy's utility for more complex problems.  While we can version artifacts, enabling detailed comparisons, our current design is not well optimized for multi-human collaboration - although, this again, points to fruitful directions for future work.}
 
One collaborator was particularly interested in understanding when humans took machine suggestions and applied them and when they ignored suggestions. A specific artifact sequence of interest began with the initial dataset, followed by wrangling transformation recommendations with a machine source. Then the recording of user actions would indicate whether the end-user applied any wrangling transformation recommendations. Finally, it concluded with any potential updates to the initial dataset. \revMR{This is yet another interesting usage scenario that not only enables us to understand a system's level of automation but, potentially defines signatures of automation per user. Moreover, it is also possible to assess whether some artifacts are modified more often than others. Collectively, these signatures could be leveraged to identify problematic features (for example, if the machine's results are constantly overwritten) or patterns of analysis behavior. }

% While~\SYSTEMNAME~can show these events in sequence, some of the temporal aspects are not fully captured by this implementation. However, this observation by our participant links work on tracing AutoML artifacts to the myriad of temporal sequence visualizations~\cite{guo:timevis_survey:2021}, which prior work in AutoML pipeline visualization has not extensively explored. 

%Our collaborators also wanted to use the artifacts to compare analyses across multiple sessions and users. While we can version artifacts, enabling detailed comparisons is presently out of scope. We see this is as a promising sign of our taxonomy's utility. Moreover, we see ample opportunities to enhance~\SYSTEMNAME~ with design alternatives proposed by prior visualization systems that compare simpler AutoML pipelines.  

\vspace{2mm}
\noindent\textbf{Comparing their system to others.} The taxonomy we developed is an amalgamation of various systems that span both human and machine processes. Our taxonomy provided a standard vocabulary for comparing these systems and reflecting on what artifacts might be missing relative to another system. For example, more recent advances in AutoML technology includes a computational budget to enable these automated processes to complete within a reasonable time frame and budgetary constraints. 
However, not all AutoML systems have such features.
Our taxonomy prompted a discussion of the design implications for our collaborator's system. They were first comforted to see that their existing system had elements that overlapped with others, but, could also see other interesting aspects that were absent in their current implementation. 

% In this way, our taxonomy provides a standardized vocabulary for such considerations and discussions. 
% Finally, our taxonomy can also facilitate conversations around what is inaccessible, which~\SYSTEMNAME~already incorporates. 


%\subsection{Expanding AutoML Trace}
%Our goal in presenting AutoML trace is not to conduct a design study nor develop a final visualization system for surfacing and tracing artifacts. 
%Our goals for developing~\SYSTEMNAME\~were formative and exploratory. This initial exploration showed that our taxonomy is useful for annotating artifacts from existing systems and leveraging them to support the design and development of an AutoML system. We believe this ability to augment the design of AutoML systems 
%We see ample opportunities for future work now that we have determined that it is both possible and useful to use our AutoML artifact taxonomy to analyze an existing system, through its APIs. We believe that it 
%is a distinct advantage of our taxonomy. Specifically, it can support both prospective ideas for system design (i.e., by showing what is possible) and also retrospectively analyze an existing system as we have done here. We were also encouraged by this initial feedback showing that~\SYSTEMNAME~prompted our collaborators to interrogate the trade-off of tasks and transfer of information between humans and the AutoML process. We will explore these promising signs in future studies that build off of the present research. 


\subsection{Summary}
In this second phase of research,  we probed the utility and ecological validity of taxonomy by collaborating with a team developing a complex AutoML system. Our formative study, supported by the~\SYSTEMNAME\ sketch demonstrates that a taxonomy is a useful boundary object to engage with a team of software and ML/AI experts designing human-ML/AI collaborative systems. It also demonstrates that traceability has valuable applications to both human-machine and human-human collaborations. While our approach does not address all of the design challenges for evolving and adaptive systems~\cite{Yang:HAI_hard:2020}, it does take preliminary steps toward doing so.
%Overall, this collective feedback shows that our taxonomy is valuable and applicable to the design and development of production systems. It also demonstrates that surfacing AutoML artifacts elicits deeper questions about automated data science processes that data visualization systems can address. While our present~\SYSTEMNAME~prototype does not answer all of these questions at this time, it does take preliminary steps toward doing so. 


%Through the development of the~\SYSTEMNAME\ interactive sketch, we demonstrate that surfacing and tracing artifacts using our taxonomy is both possible and useful to mediate discussions around design human-ML/AI collaborations. %Moreover, we also could see the value in helping designers and developers reflect on their design choices and better examine how other people would use their system.

%In this second phase of our research (\autoref{fig:artifacts}) we assess the descriptive utility of our taxonomy in a case study with a project team developing an AutoML system. In case study we have developed \SYSTEMNAME\, which to aims to riefy the abstractions of our taxonomy. 


==> tex/taxonomy_methodology_extra.tex <==
\section{EXTRA Methodology for Developing an AutoML Artifact Taxonomy}\label{taxonomy-method-extra}
%This section describes the creation of a taxonomy for classifying artifacts derived from an end-to-end AutoML workflow. Prior work by both Nickerson\textit{et al.}~\cite{Nickerson:taxonomy:2012} and Prat \textit{et al.}~\cite{Prat:taxonomy:2015} inform our taxonomy definition and development; we provide a brief description of their approach here. We then describe how we use this approach to develop our AutoML artifact taxonomy.

%We have made the supplementary materials of our approach \href{https://osf.io/3nmyj/?view_only=19962103d58b45d289b5c83421f48b36.19}{\textcolor{blue}{\texttt{available online}}} \footnote{For the review process this is an OSF view only link, meaning it does not collect any data that could deidentify reviewers}. Moreover, we reference individual items using the \textcolor{blue}{\texttt{[SM\#]}} notation; these notations are hyperlinks leading to the items themselves in an online repository. Finally, we present a brief description of individual supplementary material items at the end of this manuscript in Section~\ref{the-end}.

\subsection{Taxonomy Definition}\label{tax-defintion-extra}
%A taxonomy is a system of classification that describes an object, a living organism, a corpus of texts, or in our case, a set of artifacts, according to dimensions and characteristics. In their work, Nickerson et al.~\cite{Nickerson:taxonomy:2012} describe the differences between taxonomy and other terms that it is often confused for, such as classification, framework, or typology.  To the best of our knowledge, the visualization (vis) and human-computer interaction (HCI) communities lack a unified approach to develop taxonomies. Consequently, taxonomies that appear in the research literature vary in their development methodologies and end-result; in fact, there exists considerable variability even beyond vis and HCI~\cite{Nickerson:taxonomy:2012}. Here we have adopted an approach for taxonomy development proposed by Nickerson \textit{et al.}~\cite{Nickerson:taxonomy:2012}. 

Nickerson et al~\cite{Nickerson:taxonomy:2012} proposes uses a specific definition of a taxonomy that constitute a set of objects and taxonomic descriptors. Meta-characteristics guide the search for objects. However, there are also constraints imposed on dimensions, categories, and characteristics to ensure that the taxonomy is concise while still being usefully descriptive of the current objects under study, but also those that may be classified according to our taxonomy in the future. First, each dimension should have two or more categories. Second, each category should have two or more characteristics. If a dimension and category does not meet these requirements, then, it should not be included in in the set of taxonomic descriptors. These conditions can be expressed using  using a symbolic notation. While using this notation can add complexity, it explicates a specific set of rules that can be used to extend our current work or transfer it to an algorithmic implementation with greater ease. 

Nickerson describes a taxonomy, $T$, as follows :
\begin{equation}\label{nickerson-t}
    T = \{D,i=1,...,n | d_i = \{C_{ik},k=1,...,k_i;K \geq 2\}\}
\end{equation}

where $T$, comprises a set of \textit{\textbf{dimensions}} $D = \{d_1,....d_n\}$, where each dimensions is an aspect of an object.  Dimensions comprise a set of mutually exclusive \textit{\textbf{ characteristics}} $C = \{c_1,...,c_k\}$, where  $d_i = \{c_1,c_2,....,c_l; k \geq2\}$. Nickerson taxonomy definition states that each dimension must have at least \textit{two} characteristics, otherwise it is not concise. Moreover, an object can posess only a \textit{single characteristic per dimension}. For example, if $D_1$ has characteristics $(c_{11},c_{12})$ then some object can only poses \textit{one} of either $c_{11}$ or $c_{12}$. If this condition is not met, the taxonomy is not especially useful or robust, as it does not adequately describe or differentiate objects from one another. 
Prat \textit{et al}.~\cite{Prat:taxonomy:2015} extended on Nickerson's taxonomy definition by allowing characteristics to be grouped into categories ($Cat$). They similarly propose an extended mathematical definition for a taxonomy as:

\begin{equation}\label{pratt-t}
    T = \{D,i=1,...,n | d_i = \{Cat_{ij},j=1,...,j_i\} | 
    Cat_{i1} = \{C_{ik},k=1,...,k_i;k_i \geq 2\} \wedge \forall j \geq 2, Cat_{ij} \subset Cat_{i1}
\end{equation}
This definition proposes a two-level hierarchy, where each dimension serves as a root node ($C_{i1}$), with at least two categories ($Cat_{ij}; j \geq 1$). These categories, in turn, each contain a set of at least two characteristics ($C_{ik}; k \geq 2 $). In our work, we use Prat's definition of a taxonomy.

Both Nickerson \textit{et al.}~\cite{Nickerson:taxonomy:2012} and Prat \textit{et al.}~\cite{Prat:taxonomy:2015} contained examples of how to use their approaches to generate a taxonomy.% Nickerson emphasizes that taxonomies can be useful without necessarily being the 'best' or `correct.` They cite prior research that indicates a taxonomy is a `design search process' with an intractable solution. However, they propose five qualitative attributes that can signal their usefulness to be assessed by creators and evaluators of taxonomies. \textbf{Conciseness} such that a taxonomy contains a parsimonious and limited number of dimensions, categories, and characteristics. \textbf{Robustness} such that it can be used to differentiate between two or objects. \textbf{Comprehensiveness} such that it can be used to effectively classify all objects under consideration. \textbf{Extensibility} such that others could easily modify or add to the taxonomy beyond its immediate development. \textbf{Explainability} such that it does not describe every possible detail but is nonetheless useful to describe the overall nature of objects currently under study and other ones that may arise in the future.  
%taxonomy developed to classify a fish (object), could assign a `sea creature' dimension and a `scaled body' characteristic (among others)\footnote{The Linnaean taxonomy that classifies living things uses a more complex structure than simply a single dimensions and and characteristic. However, the physiological aspects of living organism are indeed characterized to lower levels of granularity so that biologists and others could classify existing and new organisms. The Linnaean taxonomy is also a ranked hierarchy and this is not a necessary characteristic for all taxonomies.}. 

\subsection{Taxonomy Development Methodology Details}\label{approach-method-extra}

We collected 40 research manuscripts about AutoML systems, user studies on AutoML, and finally examples of its applications. We identified and extracted artifacts from these manuscripts and developed our taxonomy over multiple iterations using a primarily empirical approach~\cite{Nickerson:taxonomy:2012} (\autoref{fig:tax_method}). An illustration of our taxonomy development is shown in~\autoref{fig:tax_iterl}; for reasons of space, the actual results are in \suppTaxSpread.

\subsubsection{Meta-characteristic and End Conditions Definitions}\label{approach-defintions-extra}
We follow Nickerson et al.'s~\cite{Nickerson:taxonomy:2012} approach. At the outset of the taxonomy development, we defined a meta-characteristic to scope the objects we wish to classify and a set of end conditions where we conclude the development process.  We define the \textbf{meta-characteristic} as :
\begin{quote}
\textit{Human or machine generated artifacts result from an end-to-end AutoML pipeline comprising preparation, analysis, deployment, communication, and governance workflow stages. We further focus on those objects that cross boundaries between human and machine processes.}
\end{quote}

Nickerson~\textit{et al.}~\cite{Nickerson:taxonomy:2012} present a comprehensive set of objective and subjective criteria for end-conditions, among which we discussed and agreed upon ahead of developing our taxonomy.

Objective end conditions stipulate that the taxonomy must be the definitions presented in~\autoref{nickerson-t} and ~\autoref{pratt-t}, which we enumerate as:
\begin{enumerate}
    \item No new dimensions, characteristics, or objects are added or modified from the previous iteration
    \item  No new dimensions, characteristics, or objects were merged and split
    \item At least one object is classified under every characteristic of each dimension
\end{enumerate}

Following each iteration, we assess whether our taxonomy is \textit{concise}, \textit{robust}, \textit{comprehensive}, \textit{extensible}, and \textit{explanatory}. While it is not possible to externally validate these qualities without additional follow-up studies, we aim for internal validity. Internally validity means that the taxonomy meets these characteristics for the objects directly under study.

\subsubsection{Iteration Details}\label{iter-details}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/tax_iter.pdf}
    \caption{Illustration of the AutoML artifact taxonomy development over time.}
    \Description{Illustration of the AutoML artifact taxonomy development over time. The figure progresses from a small table that grows in size through the different iterations, adding dimensions, categories, and measures.}
    \label{fig:tax_iterl}
\end{figure*}

Here, we describe the number of artifacts that we considered during iterative phases of our taxonomy development, the literature sources of those artifacts, and the overall approach that we took (empirical-to-conceptual or conceptual-to-empirical). We present an illustrative summary of our approach in~\autoref{fig:tax_iterl}. We remind the reader that more detailed information, including what changed and how we evaluated our end conditions, is available in~\suppTaxIter.

\vspace{1mm}
\sSec{Iterations 1 - 2} : We use an empirical-to-conceptual approach. We obtained a convenience sample for research publications through several methods. First, we collected a sample of papers known to us. Second, we used a snowball technique to find new papers from the references of these publications. In interaction 1, we started with a minimal set of 27 objects so that we could familiarize ourselves with the taxonomy methodology and have detailed discussions on how to identify characteristics that can differentiate between objects while adhering to the definitions of the taxonomy described in Nickerson \textit{et al.}~\cite{Nickerson:taxonomy:2012} and briefly summarized in Section~\ref{tax-defintion}.

\vspace{1mm}
\sSec{Iteration 3} : We used conceptual-to-empirical approach to define dimensions, categories, and characteristics. One challenge that we came upon when classifying objects in the first two iterations was that these objects exist at varying levels of granularity. For example, when referring a machine learning model choices in a component of an AutoML pipeline, some artifacts were simply `model choice', while others specified particular types of models like `linear regression' or `random forest'. Similarly, because these were technical papers, many reported on details specific to that technique. We opted to take a conceptual-to-empirical approach to help us organize these objects at a more similar level of granularity.   

\vspace{1mm}
\sSec{Iterations 4 - 5} : We returned to the set of 13 publications from which we extracted and re-coded additional artifacts based upon our conceptual-to-empirical findings. Following this re-coding, we arrived at a total of 101 objects used for both iterations. We conducted two iterations using this object set to refine taxonomy dimensions, categories, and characteristics. In iteration five, we began using our taxonomy to group individual objects into artifacts \textit{types} and \textit{groups}. Many objects could be `rolled up' into \textit{artifact types}. For example `linear regression' and `random forest' could be rolled up into `model choice'. While taxonomies focusing specifically on machine learning models could specify characteristics that differentiate these two objects, we treated both models as essentially the same type of artifact for our taxonomy.  In~\suppTaxSpread~ we have a record of how each object was rolled up; in many instances, objects were rolled up into `low-level technical details', for example, initialization parameters of a specific algorithm.

\vspace{1mm}
\sSec{Iterations 6 - 8 }: We expanded our literature sources to additional 27 literature sources. We continued to add objects and modify our dimensions, categories, and characteristics. We split these papers into groups of three, with nine papers in each iteration, to assess how much our taxonomy changed across each iteration and to assess our objective and subjective end conditions. Over these three iterations, we added 347 artifacts that we reviewed.  Although some refinements occurred, we found our taxonomy to stably incorporate new objects without affecting the taxonomic structure.
%
%\vspace{1mm}
%\sSec{Iteration 9 }: The final iteration acknowledges changes that were made when we were writing this manuscript and implementing the AutoML trace tool. These includes changes that the authors initiated as well as feedback from colleagues. 












